How Do Analysts Understand and Verify AI-Assisted Data Analyses?

Data analysis is challenging as it requires synthesizing domain knowledge, statistical expertise, and programming skills. Assistants powered by large language models (LLMs), such as ChatGPT, can assist analysts by translating natural language instructions into code. However, AI-assistant responses and analysis code can be misaligned with the analyst's intent or be seemingly correct but lead to incorrect conclusions. Therefore, validating AI assistance is crucial and challenging. Here, we explore how analysts understand and verify the correctness of AI-generated analyses. To observe analysts in diverse verification approaches, we develop a design probe equipped with natural language explanations, code, visualizations, and interactive data tables with common data operations. Through a qualitative user study (n=22) using this probe, we uncover common behaviors within verification workflows and how analysts' programming, analysis, and tool backgrounds reflect these behaviors. Additionally, we provide recommendations for analysts and highlight opportunities for designers to improve future AI-assistant experiences.

==> 0-figures-and-tables.tex <==

% \newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}

\newcommand{\interfaceFig}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{final_figures/interface7.pdf}
  \caption{\textbf{Probe Interface}. The analyst's prompt and the assistant's response are shown in the left panel. The AI's response includes its natural language explanation (A), the code and code comments involved in its calculations (B), and a description of any intermediate data (C). The original data table and intermediate data table(s) are accessible via buttons interleaved in the AI's response (D1 and E1) and when clicked point to their corresponding data pane in the right panel (D2 and E2). \rr{These panes can also be opened directly in the right panel}. In each pane, analysts can view the raw data table in the \textit{Dataset} tab with sort and filter functionality (F). Analysts can also view a visualization showing the distribution and basic descriptive statistics of each column in the \textit{Summary} tab (G).  
  % \ken{Just checking if the figure of the interface fits okay? Hard to fit everything in and it being big enough}
  }
  \Description{The screenshot of the Probe Interface web page with double column design. The page consists of two large main content areas with the chatbot interface on the left and the data tables displayed on the right. The screenshot is labeled with letters A to G that are used to describe the different features in the figure caption.}
  \label{fig:interface}
\end{figure*}
}

\newcommand{\interfaceAllFig}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{final_figures/fullinterface.pdf}
  \caption{\textbf{An example study task}. We include the description of the analysis goal and dataset in the left side-panel.}
  \Description{}
  \label{fig:interfaceAll}
\end{figure*}
}

\newcommand{\artifactsFig}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.93\linewidth]{final_figures/artifacts5.pdf}
  \caption{Both data and procedure artifacts were used to support \rr{participant's primary behaviors}. For each type of behavior illustrated in Fig.~\ref{fig:workflows}, we tally the unique artifacts involved, counting each artifact once per occurrence in a behavior. This distribution shows that participants extensively used data artifacts to support \processworkflows~and used procedure artifacts to support \dataworkflows~ (Top). The intermediate data, original, data, code, and natural language explanation were all pivotal for analysts' to notice an issue (Bottom).
  }
  \Description{Two vertically stacked horizontal bar charts of counts of artifacts used in data and procedure-oriented workflows. The top one shows the total counts used in the data and procedure-oriented behaviors, and the bottom one shows the counts used in different behaviors that helped participants notice an issue.}
  \label{fig:artifacts}
\end{figure*}
}

\newcommand{\workflowsFig}{
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{final_figures/workflows5.pdf}
  \caption{\textbf{\rr{Participants often followed \textit{procedure-oriented behaviors}.}} 
  % We count occurrences of activities across all verification processes observed in our study. 
  % \teal{Data Only} (using data artifacts only) and ~\blue{Data + Procedure} (using procedure artifacts to support a focus on the data) are \dataworkflows~. Meanwhile, \red{Procedure Only} (using procedure artifacts only) and \orange{Procedure + Data} (using data artifacts to support a focus on the procedure) are \processworkflows~. Finally, \yellow{Notice} is when participants noticed an issue in the data/AI's work that might have affected the correctness of the task. 
  % \tim{I'm assuming procedure means code here? make sure to clarify this. is this 1 to 1? if yes, why not use Code + Data etc?  }
  }
  \Description{Bar chart of the counts of different behaviors. 'Data Only' has a count of 17, 'Data + Procedure' has a count of 13, 'Procedure Only' has a count of 9, 'Procedure + Data' has a count of 48, and 'Notice' has a count of 38.}
  \label{fig:workflows}
\end{figure}
}


\newcommand{\tableDefs}{
\begin{table}[t]
\small 
    \centering
    \begin{tabular}{lp{5.7cm}}
        \toprule
        Label & Definition \\
        \midrule
        \start~& Start of a verification workflow \\
        \dataonly~& Using data artifacts only\\
        \data~& Mainly focusing on the data and using procedure artifacts as secondary support \\
        \processonly~& Using procedure artifacts only \\
        \process~& Mainly focusing on the procedure and using data artifacts as secondary support \\
        \notice~& Noticing an issue that may affect the correctness of the AI-generated result \\
        \confirm~& Confirming or rejecting that the AI-generated analysis has an error\\
        

        \bottomrule
    \end{tabular}
    \caption{\textbf{Definition of labels used to annotate participants' verification workflows.} \dataonly~and~\data~are behaviors under \textit{data-oriented behaviors}~while \processonly~and~\process~are behaviors within \textit{procedure-oriented behaviors}.}
    \label{tab:labeldefs}
\end{table}
}

% \newcommand{\tableWorkflows}{
% \begin{table} 
%     \small
 
% \begin{tabular}{llllll}
%     \toprule
%     Behavioral Patterns & Count & Occurrences in Observed Verification Workflows \\
%     \midrule
%     \pdShort---\noticeShort---\dShort & 9 & T1 [P1], T2 [P5, P12], T4 [P2], T5 [P4], T6 [P14], T8 [P22], T9 [P6], T10 [P22]\\
%     \pdShort---\noticeShort---\pdShort & 6 & T3 [P5, P12], T6 [P4, P14], T7 [P12], T10 [P20] \\
%     \pdShort---\noticeShort---\confirmShort& 5 & T1 [P7], T2 [P2], T4 [P6], T5 [P10, P14] \\
%     \pdShort---\noticeShort---\dpShort & 3 & T2 [P1], T4 [P21], T10 [P13] \\
%     \pShort---\noticeShort---\pdShort & 3 & T5 [P4, P8], T8 [P11]\\
%     \dpShort---\noticeShort---\dShort & 3 & T4 [P15], T7 [P16], T9 [P9] \\
%     \dpShort---\noticeShort---\confirmShort & 2 & T2 [P1], T10 [P13] \\
%     \pShort---\noticeShort---\pShort & 2 & T7 [P4, P6] \\
%     \bottomrule
% \end{tabular}
%   \caption{\textbf{Participants' Behaviors Around Noticing an Issue.} We report patterns around noticing an issue that occurred more than once in our study. 
%   % In this table, \pShort is \processonly~; \pdShort~is \process~; \dShort~is \dataonly~; \dpShort~is \data~; \noticeShort~is \notice~; and \confirmShort~is~\confirm. 
%   Participants often followed \processworkflows~before noticing an issue and used a variety of \dataworkflows~and\processworkflows~afterwards to validate their concerns.}
%   \label{tab:freq-of-workflows}
% \end{table}
% }


\newcommand{\tableWorkflows}{
\begin{table} 
    \small
 
\begin{tabular}{llp{4.9cm}}
    \toprule
    Patterns & Count & Occurrences in Verification Workflows \\
    \midrule
    \pdShort---\noticeShort---\dShort & 9 & T1 [P1], T2 [P5, P12], T4 [P2], T5 [P4], T6 [P14], T8 [P22], T9 [P6], T10 [P22]\\
    \pdShort---\noticeShort---\pdShort & 6 & T3 [P5, P12], T6 [P4, P14], T7 [P12], T10 [P20] \\
    \pdShort---\noticeShort---\confirmShort& 5 & T1 [P7], T2 [P2], T4 [P6], T5 [P10, P14] \\
    \pdShort---\noticeShort---\dpShort & 3 & T2 [P1], T4 [P21], T10 [P13] \\
    \pShort---\noticeShort---\pdShort & 3 & T5 [P4, P8], T8 [P11]\\
    \dpShort---\noticeShort---\dShort & 3 & T4 [P15], T7 [P16], T9 [P9] \\
    \dpShort---\noticeShort---\confirmShort & 2 & T2 [P1], T10 [P13] \\
    \pShort---\noticeShort---\pShort & 2 & T7 [P4, P6] \\
    \bottomrule
\end{tabular}
  \caption{\textbf{Participants' behaviors around noticing an issue.} We report patterns around noticing an issue that occurred more than once in our study. 
  % In this table, \pShort is \processonly~; \pdShort~is \process~; \dShort~is \dataonly~; \dpShort~is \data~; \noticeShort~is \notice~; and \confirmShort~is~\confirm. 
  Participants often followed \processworkflows~before noticing an issue and used a variety of \dataworkflows~and~\processworkflows~afterwards to validate their concerns.}
  \label{tab:freq-of-workflows}
\end{table}
}


\newcommand{\tableAllWorkflows}{
\begin{table*} 
    \small
 
\begin{tabular}{llllll}
\toprule
Verification Processes & Count & Occurrences \\
    \midrule
    \tsShort---\pdShort---\confirmShort & 11 & T4 [P10], T6 [P10, P20, P8], T9 [P10, P11, P21], T3 [P2, P22], T8 [P7], T7 [P8] \\
    \tsShort---\pdShort---\noticeShort---\dShort---\confirmShort & 7 & T1 [P1], T2 [P12, P5], T4 [P2], T8 [P22], T10 [P22], T9 [P6] \\
    \tsShort---\pdShort---\noticeShort---\confirmShort & 5 & T5 [P10, P14], T2 [P2], T4 [P6], T1 [P7] \\
    \tsShort---\pdShort---\noticeShort---\pdShort---\confirmShort & 5 & T3 [P12, P5], T7 [P12], T10 [P20], T6 [P4] \\
    \tsShort---\dpShort---\noticeShort---\dShort---\confirmShort & 3 & T4 [P15], T7 [P16], T9 [P9] \\
    \tsShort---\pdShort---\noticeShort---\dpShort---\noticeShort---\confirmShort & 2 & T2 [P1], T10 [P13] \\
    \tsShort---\pShort---\noticeShort---\pdShort---\confirmShort & 2 & T8 [P11], T5 [P8] \\
    \tsShort---\dpShort---\confirmShort & 2 & T5 [P17], T1 [P20] \\
    \tsShort---\pShort---\noticeShort---\pShort---\confirmShort & 2 & T7 [P4, P6] \\
    \tsShort---\dpShort---\noticeShort---\pdShort---\confirmShort & 1 & T3 [P1] \\
    \tsShort---\pdShort---\dShort---\confirmShort & 1 & T9 [P13] \\
    \tsShort---\pdShort---\noticeShort---\pdShort---\noticeShort---\dShort---\confirmShort & 1 & T6 [P14] \\
    \tsShort---\dShort---\dpShort---\confirmShort & 1 & T1 [P15] \\
    \tsShort---\pShort---\noticeShort---\dpShort---\confirmShort & 1 & T6 [P17] \\
    \tsShort---\pdShort---\runOutOfTimeShort & 1 & T9 [P18] \\
    \tsShort---\dShort---\confirmShort & 1 & T8 [P19] \\
    \tsShort---\dpShort---\pdShort---\noticeShort---\pShort---\pdShort---\confirmShort & 1 & T9 [P19] \\
    \tsShort---\pdShort---\noticeShort---\dpShort---\confirmShort & 1 & T4 [P21] \\
    \tsShort---\dShort---\noticeShort---\dpShort---\runOutOfTimeShort & 1 & T7 [P3] \\
    \tsShort---\pShort---\noticeShort---\pdShort---\noticeShort---\dShort---\confirmShort & 1 & T5 [P4] \\
    \tsShort---\pdShort---\runOutOfTimeShort & 1 & T8 [P5] \\
    \tsShort---\dShort---\noticeShort---\pdShort---\confirmShort & 1 & T10 [P7] \\
    \bottomrule
\end{tabular}
  \caption{\textbf{All Participants' Behaviors in Their Workflows.} \runOutOfTimeShort~is when the participant ran out of time on the task or was unable to confirm or reject the AI-generated output has an error. In 52 verification workflows, we observed 3 such cases.}
  \label{tab:all-workflows}
\end{table*}
}

\newcommand{\casesFig}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{final_figures/cases3.pdf}
  \caption{We show examples of interesting end-to-end verification \rr{workflows} and associated artifacts using our labels in Table~\ref{tab:labeldefs}. The labels help get a sense of the overall workflow and capture relevant behavioral patterns. For example, in T5, we observed P4 starting out (\start~) focusing only on the natural language explanation (\processonly~) before noticing an issue (\notice~) from the explanation. Their behavior then shifts slightly as they include data artifacts (\process~) before noticing a subsequent issue in the code (\notice~). Finally, they check the result data (\dataonly~) to confirm an error in the AI's analysis (\confirm~). Overall, we observed 52 verification \rr{workflows} in our study (39 of which involved errors) with an average length of 4.40 (std=1.42) labels. Four of these had two \notice~patterns occur, 30 had one~\notice~pattern occur and the rest had none.
  }
  \Description{Three linear flow charts from left to right connected by arrows for a participant and task pair. The first row is for P1, T2, the second row for P4, T5, and the third row for P9, T9. Behaviors are written in blocks connected by arrows. Above the blocks are different artifacts that were used for that behavior. The start states are all 'Start', and the end states are all 'Confirm'.}
  \label{fig:cases}
\end{figure*}
}

\newcommand{\motivateFig}{
\begin{figure*}[h!]
  \centering
  \includegraphics[width=0.92\linewidth]{final_figures/motivate3.pdf}
  
  \caption{\textbf{Analysts may now need to understand and verify AI-assisted analyses}. In traditional analysis workflows, analysts specify and execute their data operations using tools such as computational notebooks (A) or spreadsheets (B). Engaged in these operations, analysts are familiar with the process and results of their work (e.g., reports, code, tables, and visualizations). However, with AI-assisted analysis, analysts can convey their intentions using natural language (e.g., "\textit{How many items purchased within the month of November were returned to the seller?}"). The AI assistant handles the task of specifying and performing the data operations. This shift requires analysts, including those who may not be familiar with the underlying execution language the assistant uses, to understand and verify the process and results of the assistant (C). In this paper, we study the workflows analysts with varied backgrounds use to understand and verify AI-assisted data analyses. 
  }
  % \textbf{Example: Traditional vs. AI-Assisted Data Analysis}. Jane writes her analysis in a computational notebook and is able to write code to check her data and see her steps in the calculation. Meanwhile, Alex leverages an AI assistant to generate the analysis based on a natural language prompt but must validate the AI's work.}
  \Description{Three images labelled A, B, and C showing the screenshots of the the data analysis tools. A and B are on the left side under the title "Traditional Data Analysis". C is on the right side with the title "AI-Assisted Data Analysis". Image A shows the partial interface of working with spreadsheets. Image B shows the partial interface of a Jupyter notebook during data analysis. Image C shows the chatbot interface between a user and an AI assistant where the user asks a question and the AI produces the data analysis output. All three images are labelled with emojis of different people.}
  \label{fig:motivate}
\end{figure*}
}


\newcommand{\tableParticipants}{
\begin{table*}
    \small
 
  \begin{tabular}{llrlp{2.6cm}lp{1.7cm}}
    \toprule
    \textbf{PID} & \textbf{Role} & \textbf{Exp.} & \textbf{Primary Analysis Tools} & \textbf{Analysis Frequency} & \textbf{Coding Comfort} & \textbf{Tasks Shown} \\
    \midrule
    P01 & Data Scientist & 6 Y  & Code/Computational Notebooks  & Daily & Very Comfortable & [T1, T2, T3] \\
    P02 & Software Engineer & 4 Y & Data Visualization Tools & Daily & Very Comfortable  & [T2, T3, T4]\\
    P03 & Consultant &  26 Y & Spreadsheets & Daily & Somewhat Comfortable & [T7]\\
    P04 & Data Analyst & 10 Y & Data Visualization Tools & Weekly & Somewhat Comfortable  & [T5, T6, T7]\\
    P05 & Software Engineer & 10 Y & Code/Computational Notebooks & Weekly & Very Comfortable & [T2, T3, T8]\\
    P06 & Program Manager &  12 Y&  Spreadsheets & Weekly & Very Comfortable & [T4, T7, T9]\\
    P07 & Program Manager &  6 Y& Spreadsheets  & Monthly & Neutral & [T1, T8, T10] \\
    P08 & Software Engineer & 7 Y& Code/Computational Notebook & Weekly & Very Comfortable & [T5, T6, T7]\\
    P09 & Program Manager &  3 Y& Spreadsheets & Daily & Neutral & [T9]\\
    P10 & Tech. Strategist & 15 Y&  Spreadsheets & Monthly & Neutral & [T4, T5, T6, T9] \\
    P11 & Program Manager &  11 Y&  Data Visualization Tools & Daily & Somewhat Comfortable & [T8, T9]\\
    P12 & Program Manager & 5 Y&  Spreadsheets & Daily & Neutral  & [T2, T3, T7] \\
    P13 & Cloud Architect & 5 Y&  Spreadsheets & Daily & Somewhat Comfortable  & [T9, T10] \\
    P14 & Program Manager & 0.5 Y& Code/Computational Notebook & Weekly & Very Comfortable  & [T5, T6]\\
    P15 & Program Manager & 10 Y& Spreadsheets & Daily & Somewhat Comfortable  & [T1, T4]\\
    P16 & Program Manager & 15 Y& Spreadsheets & < Monthly & Never Coded Before & [T7] \\
    P17 & Software Engineer & 15 Y & Code/Computational Notebook & Weekly & Very Comfortable & [T5, T6] \\
    P18 & Program Manager & 7 Y& Data Visualization Tools & Daily & Somewhat Comfortable  & [T9] \\
    P19 & Finance Manager & 13 Y& Spreadsheets & Daily & Neutral  & [T8, T9]\\
    P20 & Program Manager & 3 Y& Data Visualization Tools & Daily & Somewhat Comfortable & [T1, T6, T10]\\
    P21 & Customer Manager & 8 Y& Spreadsheets & Daily & Very Comfortable  & [T4, T9]\\
    P22 & Architect & 5 Y & Code/Computational Notebook & Weekly & Very Comfortable  & [T3, T8, T10]\\
    \bottomrule
  \end{tabular}
  \caption{Participants reported using a variety of tools to perform data analysis in their normal workflows and came from a variety of roles and teams. Over half (13/22) of the participants reported being somewhat comfortable (knowing programming basics and can write simple programs) or less with programming.}
   \label{tab:participants}
\end{table*}
}

\newcommand{\tableTasks}{
\begin{table*}[t]
    \small
 
  \begin{tabular}{lp{1.1cm}p{5.7cm}p{6.0cm}p{1.6cm}}
    \toprule
    \textbf{TID} & \textbf{Task} & \textbf{Natural Language Prompt} &  \textbf{\rr{Error Type and Summary}} &\textbf{PIDs} \\
    \midrule
    T0~\cite{Tutorial} & \raggedright Tutorial & What is the least possible age of students having high adaptivity?  & \textit{Data}---AI and took the minimum of age-range by alphanumeric order.  &  Everyone \\
    \midrule
    T1~\cite{AmazonOrders} & \raggedright Amazon Orders & How many items purchased within the month of November were returned to seller?  & \textit{Prompt}---AI counted the quantity of products returned, instead of the number of unique products.&  P1, P7, P15, P20 \\ 
    \midrule
    T2~\cite{BigBasket} & \raggedright Big Basket1& Show a list of the top five rated Nivea products. & \textit{Data}---AI missed "Nivea Men" products in the data. &  P1, P2, P5, P12 \\
    \midrule
    T3~\cite{BigBasket} & \raggedright Big Basket2&  How expensive are gourmet products compared to beverage products in average? Show the value as a percentage of beverage products. & \textit{Correct} &    P1, P2, P5, P12, P22 \\
    \midrule
    T4~\cite{Bollywood} & \raggedright Bollywood & Show the top 5 movies with the highest percentage return on investment. & \textit{Calculation}---AI mentioned but did not ignore rows with bad budget values. The intern did not filter for only Bollywood movies. &  P2, P6, P10, P15, P21  \\
    \midrule
    T5~\cite{Flights} & \raggedright Flights1& What is the city that has the highest number of incoming flights? How many incoming flights does each airline have for that city with one week left until departure? Show the city name, airline and number of incoming flights. & \textit{Calculation \& Data}---AI performed the wrong order of filtering. It also incorrectly counted incoming flights based on booking rows rather than by unique flight codes.  &  P4, P8, P10, P14, P17\\
    \midrule
    T6~\cite{Flights} & \raggedright Flights2&  What is the least expensive time of the day to depart to Chennai in Economy class across all airlines? Show the time of the day and the fare price for each airline. &\textit{Propmt}---For each airline, the AI calculated the minimum price of all flights during a time of day rather than the minimum of the average price of flights during a time of day. &  P4, P8, P10, P14, P17, P20 \\
    \midrule
    T7~\cite{Hotels} & \raggedright Hotels& Which hotels had a worse ranking this year than in 2021? Show the hotel name, location and the difference in ranking from last year. & \textit{Data}---AI misinterpreted a "2021" flag column as representing the rank in 2021. &  P3, P4, P6, P8, P12, P16  \\
    \midrule
    T8~\cite{MovieContent} & \raggedright Movie Content& What is the number of shows viewed in distinct languages within each genre as a percentage of the total number of shows within each genre? Show the genres as an index and languages as columns & \textit{Calculation}---Inverted the percentage calculation. Summing across genres for a given language should add up to 100 but the AI's calculation resulted in summing across languages for a genre adding up to 100. &  P5, P7, P11, P19, P22 \\
    \midrule
    T9~\cite{Netflix} & \raggedright Netflix& Who is the actor who worked with the same director the most? &  \textit{Correct} &   P6, P9-11, P13, P18, P19, P21  \\
    \midrule
    T10~\cite{TV} & \raggedright TV&What are the top 5 most selling television frequencies? Show the frequencies with their counts &  \textit{Data}---The AI cleaned dirty frequency data but it neglected correct data that existed in other columns. &  P7, P13, P20, P22 \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{User Study Tasks.} These tasks and natural language prompts were derived from Yin et al.~\cite{Yin2022NaturalLT}. The prompts were written by data scientist annotators, who were instructed
  % to phrase their instructions in a manner they naturally prefer while communicating with an AI system. They were also asked 
  to be natural, concise, and avoid unnecessary elaborations. AI errors encompassed poor interpretations of the prompt and data, and incorrect calculations. Although creating more precise prompts can potentially reduce errors, our study is not centered on this aspect. 
  % The verification of AI's generations is relevant regardless of the exactness in the prompt formulation.
  }
   \label{tab:tasks}
\end{table*}
}






==> 0-macros.tex <==

\newcommand{\other}[1]{{\color{blue}{#1}}}
\newcommand{\ken}[1]{{\color{orange}{Ken: #1}}}
\newcommand{\chenglong}[1]{{\color{olive}{Chenglong: #1}}}
\newcommand{\steve}[1]{{\color{green}{Steve: #1}}}
\newcommand{\anna}[1]{{\color{blue}{Anna: #1}}}
\newcommand{\tim}[1]{{\color{magenta}{Tim: #1}}}
\newcommand{\rr}[1]{{\color{black}{#1}}}


\newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1.}}}
\newcommand{\yhdr}[1]{\vspace{1.7mm}\noindent{{\it #1.}}}

\newcommand{\nparticipants}{22\xspace}
\newcommand{\codeInterpreter}{Code Interpreter\xspace}


\usepackage{comment} % for long comments
\usepackage{xspace}
% For related work 
\newcommand{\interfont}{\fontfamily{cmss}\selectfont}

% For lab findings

\newcommand{\theme}[1]{\vspace{-1pt}\subsubsection{#1} }
\newcommand{\groupingtheme}[1]{\subsubsection{\textbf{#1}} }


%For terms
\def\processworkflow{procedure-oriented \behavior}
\def\dataworkflow{data-oriented \behavior}
\def\processworkflows{procedure-oriented \behaviors}
\def\dataworkflows{data-oriented \behaviors}
\newcommand{\process}[1]{\orange{Procedure + Data}\xspace}
\newcommand{\processonly}[1]{\red{Procedure Only}\xspace}
\newcommand{\data}[1]{\blue{Data + Procedure}\xspace}
\newcommand{\dataonly}[1]{\teal{Data Only}\xspace}
\newcommand{\notice}[1]{\yellow{Notice}\xspace}
\newcommand{\confirm}[1]{\green{Confirm}\xspace}
\newcommand{\start}[1]{\gray{Start}\xspace}


\newcommand{\shortquote}[1]{``\emph{#1}''}
\newcommand{\longquote}[1]{\vspace{-1pt}\begin{quote}``\emph{#1}''\end{quote}}

\usepackage{xcolor}
% \definecolor{redbg}{RGB}{255,207,201}
% \definecolor{redtxt}{RGB}{177,2,2}
% \definecolor{orangebg}{RGB}{255,200,170}
% \definecolor{orangetxt}{RGB}{117,56,0}
% \definecolor{yellowbg}{RGB}{255,229,160}
% \definecolor{yellowtxt}{RGB}{71,56,33}
% \definecolor{bluebg}{RGB}{191,225,246}
% \definecolor{bluetxt}{RGB}{10,83,168}
% \definecolor{tealbg}{RGB}{198,219,225}
% \definecolor{tealtxt}{RGB}{33,90,108}
% \definecolor{greenbg}{RGB}{212,237,188}
% \definecolor{greentxt}{RGB}{17,115,75}


\definecolor{redbg}{RGB}{255,207,201}
\definecolor{redtxt}{RGB}{177,2,2}
\definecolor{orangebg}{RGB}{255,200,170}
\definecolor{orangetxt}{RGB}{117,56,0}
\definecolor{yellowbg}{RGB}{255,229,160}
\definecolor{yellowtxt}{RGB}{71,56,33}
\definecolor{bluebg}{RGB}{191,225,246}
\definecolor{bluetxt}{RGB}{10,83,168}
\definecolor{tealbg}{RGB}{198,219,225}
\definecolor{tealtxt}{RGB}{33,90,108}
\definecolor{greenbg}{RGB}{212,237,188}
\definecolor{greentxt}{RGB}{17,115,75}
\definecolor{graybg}{RGB}{217, 217, 217}
\definecolor{graytxt}{RGB}{51, 51, 51}



\usepackage{soul}
% \newcommand{\hlc}[2][yellow]{{%
%                   \colorlet{foo}{#1}%
%                   \sethlcolor{foo}\hl{#2}}%
% }

\newcommand{\hlc}[3][yellow]{{%
                  \colorlet{foo}{#1}%
                  \sethlcolor{foo}\color{#2}\hl{#3}}%
}

\newcommand\red[1]{\hlc[redbg]{redtxt}{#1}}
\newcommand\orange[1]{\hlc[orangebg]{orangetxt}{#1}}
\newcommand\yellow[1]{\hlc[yellowbg]{yellowtxt}{#1}}
\newcommand\blue[1]{\hlc[bluebg]{bluetxt}{#1}}
\newcommand\teal[1]{\hlc[tealbg]{tealtxt}{#1}}
\newcommand\green[1]{\hlc[greenbg]{greentxt}{#1}}
\newcommand\gray[1]{\hlc[graybg]{graytxt}{#1}}

\newcommand\forcespace[1]{~#1~}


\newcommand\dpShort{\hlc[bluebg]{bluetxt}{~DP~}}
\newcommand\dShort{\hlc[tealbg]{tealtxt}{~D~}}
\newcommand\pShort{\hlc[redbg]{redtxt}{~P~}}
\newcommand\pdShort{\hlc[orangebg]{orangetxt}{~PD~}}
\newcommand\noticeShort{\hlc[yellowbg]{yellowtxt}{~N~}}
\newcommand\runOutOfTimeShort{\hlc[graybg]{redtxt}{~R~}}
\newcommand\confirmShort{\hlc[greenbg]{greentxt}{~C~}}
\newcommand\tsShort{\hlc[graybg]{graytxt}{~S~}}


% We observed two types of patterns

% We observed high level pattern

% who how and what
% For lab findings
\def\behavior{behavior\xspace}
\def\behaviors{behaviors\xspace}
\def\rqWorkflows{What patterns of \behaviors do analysts follow in a verification workflow?\xspace}
\def\rqArtifacts{What artifacts do analysts use and for what purposes?\xspace}
\def\rqBackground{How are analysts' backgrounds reflected in their behaviors and artifact usage?\xspace}




==> 1-abstract.tex <==
\begin{abstract}
Data analysis is challenging as it requires synthesizing domain knowledge, statistical expertise, and programming skills. Assistants powered by large language models (LLMs), such as ChatGPT, can assist analysts by translating natural language instructions into code. However, AI-assistant responses and analysis code can be misaligned with the analyst's intent or be seemingly correct but lead to incorrect conclusions. Therefore, validating AI assistance is crucial and challenging. Here, we explore how analysts understand and verify the correctness of AI-generated analyses. To observe analysts in diverse verification approaches, we develop a design probe equipped with natural language explanations, code, visualizations, and interactive data tables with common data operations. Through a qualitative user study (n=22) using this probe, we uncover common behaviors within verification workflows and how analysts' programming, analysis, and tool backgrounds reflect these behaviors. Additionally, we provide recommendations for analysts and highlight opportunities for designers to improve future AI-assistant experiences.
\end{abstract}



==> 2-intro.tex <==
% \tim{overall this looks good in terms of organization and argument}

\motivateFig
\section{Introduction}
\label{sec:intro}
Data analysis is challenging as practitioners must synthesize domain knowledge with computational expertise to draw reliable conclusions. For practitioners, computational challenges may act as a barrier to exploring alternative and valid analysis decisions, and therefore conducting robust analyses~\cite{Liu2020UnderstandingTR, Liu2019PathsEP}.

Improved capabilities of large language models (LLMs) for general~\cite{Chen2021EvaluatingLL, Bubeck2023SparksOA, Chowdhery2022PaLMSL}, data science ~\cite{Lai2022DS1000AN, Yin2022NaturalLT, Chandel2022TrainingAE}, and visualization~\cite{Dibia2023LIDAAT} programming tasks suggest LLM-based analysis assistants as a promising solution, enabling data analysts to \textit{execute} and \textit{automate} their analyses. Given the widespread deployment of assistants such as OpenAI's \codeInterpreter ~\cite{openai_codeinterpreter}, there is an emerging paradigm in how analysts perform analyses. Rather than formulate the exact transformations and operations in an analysis, analysts specify their analysis question through a natural language intent~(Fig.~\ref{fig:motivate} right)~\cite{Liu2023WhatIW}. The AI assistant then performs the analysis task, writes code to understand the data, makes the necessary data transformations, and interprets the results. Since many analysis tasks are time-consuming~\cite{Chattopadhyay2020WhatsWW, Kandogan2014FromDT, Kandel2012EnterpriseDA, Liu2020UnderstandingTR},  even for analysts well-versed in programming, natural language interactions can be more efficient especially when abstraction of the intent is possible. Furthermore, this natural language communication can broaden the usability of AI analysis tools, making them accessible even for analysts who are non-expert programmers~\cite{Ragavan2022GridBookNL}.

% Such assistants can not only speed up their process~\cite{Vaithilingam2022ExpectationVE, Liang2023UnderstandingTU, Ziegler2022ProductivityAO} but also point insights in the data~\cite{Dibia2023LIDAAT}.
% \tim{You can also argue that many data analysis tasks are time consuming even for people who could code in principle. natural language interactions can be more efficient, especially when abstraction is possible, and that makes this attractive. being more inclusive to non-expert-analysts is another possibility.}

Yet, a significant challenge remains. AI-based assistants, while powerful, can misinterpret user intentions (see Fig.~\ref{fig:motivate})
% (e.g., \textit{filtering first then calculating the average vs. calculating the average first then filtering} \steve{this isn't really an intention misinterpretation but rather a wrong execution, it should be something like 'show me the top sales people' and it shows the people that have the most absolute sales, but not the most monetary sales})
~\cite{Liang2023UnderstandingTU, Xu2021InIDECG, Jiang2022DiscoveringTS} or make seemingly correct erroneous outputs~\cite{Bender2021OnTD, Ji2022SurveyOH}. Since misinterpretations is inherent in the flexibility of natural language communication~\cite{Liu2023WhatIW, Ragavan2022GridBookNL, Setlur2022HowDY}, errors from existing AI-based assistants are likely to persist no matter what the underlying LLM is. Moreover, because conclusions from data analyses often inform high-impact decisions in science~\cite{Baker20161500SL, Aarts2015EstimatingTR}, business~\cite{Kandel2012EnterpriseDA, Kim2018DataSI, Kim2016TheER}, and government~\cite{Hardy2017OpeningUG, Ubaldi2013OpenGD}, it is important for users of AI-based analysis assistants to critically reflect on the assistant’s outputs~\cite{Ragavan2022GridBookNL}. In this new paradigm, analysts' focus now shifts from writing and validating their own analyses to understanding and evaluating the analyses generated by AI assistants~\cite{Liang2023UnderstandingTU}. This can be challenging as existing AI assistants lack verification support~\cite{Ragavan2022GridBookNL, Sarkar2022WhatII} and even experts can be susceptible to automation bias and overreliance~\cite{Wickens2015ComplacencyAA, Parasuraman2010ComplacencyAB}.

% Prior work in the Human-Centered Explainable AI community explored ways to provide the user with a better understanding of the AI system. Notably, Sun et al.~\cite{Sun2022InvestigatingEO} explored AI explainability in AI-code assistants. Through workshops with profession software engineers, they identified 11 explainability needs and proposed four 

Recent work in the HCI community explored ways to provide the user with a better understanding of LLM-generated outputs, including those from AI-based code assistants~\cite{Sun2022InvestigatingEO, Vasconcelos2023GenerationPA}. However, these studies focus only on programmers and not the specific domain of data analysis, missing a significant portion of data analysts~\cite{Crisan2020PassingTD, Liu2020UnderstandingTR}. Since data analysis involves iteratively making sense of the underlying data~\cite{Koesten2019TalkingDU, Pirolli2007TheSP, Klein2007ADT}, analysts must juggle their mental model of the data in addition to their understanding of the AI's procedure. There is limited insight into how analysts with different programming skills and computational reasoning abilities go about this process. 
Current code assistants such as Open AI's Code Interpreter~\cite{openai_codeinterpreter} present these steps in natural language, Python code, code comments, and code execution outputs. It is unclear to what extent these interface affordances are helpful and how analysts use these different sources of information for accessing the correctness of AI-generated analyses. 

In this work, we build on the perspective of recent works in Human-Centered Explainable AI (HCXAI)~\cite{Ehsan2021ExplainabilityPB, Liao2020QuestioningTA, Liao2021HumanCenteredEA, Kim2022HelpMH} in that users' needs to understand AI-generated outputs are dependent on their backgrounds, social, and organizational contexts; we focus on data analysts as they understand AI-assisted analyses. We study the verification workflows of analysts, how different backgrounds may influence analysts' approaches, and opportunities to improve this experience. We aim to guide the design of AI assistants that empower analysts to critically reflect on AI-generated outputs. 

To explore analysts' behaviors and elicit feedback for design opportunities, we developed a prototype interface that not only includes the AI's code, code comments, and natural language explanation but also additional interactive data tables and summary visualizations (Sec.~\ref{sec:method}). This design accommodated a broad spectrum of potential artifacts that analysts may employ during verification, facilitating the observation of naturally emerging workflows.
% \tim{it's not motivated yet why this is exciting and important. I believe you have all these because they represent all the possible artifacts that could be used for validation? in the abstract you highlighted the disentangling between information and interaction as a strength but that's not included in intro and explained yet.}\ken{TODO: motivate probe} \steve{I agree with Tim on this...} 
Analysts could access intermediary data tables that let them filter, search, and sort for values to explore the data and verify the AI-generated output. Using our tool as a probe, we conducted a qualitative study with \nparticipants professional analysts (Sec.~\ref{sec:study}). We asked participants to verify AI-generated analyses that involved sequences of data transformations covering a range of real-world datasets (Table~\ref{tab:tasks}). These generated analyses were in response to high-level analysis queries written by data scientists~\cite{Yin2022NaturalLT} which were presented to participants as prompts written by an intern.

We find analysts often started their verification workflows with \textit{procedure-oriented} behaviors (answering \shortquote{what did the AI do?}) and shifted to \textit{data-oriented} behaviors (answering \shortquote{does the [resulting] data make sense?}) once they noticed issues in the AI-generated output (Table~\ref{tab:freq-of-workflows}). Analysts adopted procedure-oriented behaviors to get a high-level understanding of the analysis steps and confirm low-level details in the data operations. Meanwhile, analysts adopted data-oriented behaviors to make sense of the data. 
% two prevailing \behaviors~in their verification workflows: one that is \textit{procedure-oriented} (answering \shortquote{what did the AI do?}), and another that is \textit{data-oriented} (answering \shortquote{does the data make sense?}). Notably, we observed analysts frequently oscillated between these \behaviors, shifting especially when they noticed issues in the AI-generated output (Table~\ref{tab:freq-of-workflows}).
Notably, \textit{data artifacts} (i.e., the data tables and summary visualizations) were often vital as secondary support in \textit{procedure-oriented} \behaviors, and vice versa for \textit{procedure artifacts} (i.e., the natural language explanation and code/code comments) (Fig.~\ref{fig:artifacts}). 

Based on these findings (Sec.~\ref{sec:results}), we make recommendations to end-user analysts interacting with AI-based analysis assistants (Sec.~\ref{sec:discussion_impl_analyst}). Additionally, we discuss  implications for system designers (Sec.~\ref{sec:discussion_impl_designers}). These center around fluidly connecting data-oriented and procedure-oriented artifacts, communicating data operations and AI's assumptions about the data, and incorporating AI guidance into verification workflows.


This paper contributes the following:
\begin{enumerate}

% \item A categorization of data analysis planning suggestion content 
% \item An open-source data analysis assistant interface prototype integrated into JupyterLab
\item Findings from a user study using our design probe that uncover common behavioral patterns in the verification of AI-generated analyses,
\item A set of implications for end-user analysts interested in AI-assisted data analysis, paired with design implications for tool builders to improve verification workflows.
\end{enumerate}

==> 3-motivating-example.tex <==

\section{Motivating Example}
To illustrate the potential errors and verification workflows in AI-assisted analyses, we compare three hypothetical analysts working on the same analysis question~(Fig.~\ref{fig:motivate}). This scenario highlights the workflow differences between traditional and AI-assisted data analysis. Jane, Kate, and Alex are data analysts at a company that sells products on a popular e-commerce platform. They want to assess how many products may have quality control issues as the year draws to a close. Specifically, they want to find out how many distinct products bought in November were later returned.
% \tim{this might be detail oriented but doesn't it make more sense to look at the volume of returned items rather than the set of unique products that was returned?} 
To perform this analysis, they have a dataset of product orders where each row is a unique order for a product and its associated order status. The dataset contains the following key columns:
\begin{itemize} 
  \item \textbf{order\_date}: the date which the order was placed
  \item \textbf{sku}: a unique identified for the product
  \item \textbf{quantity}: the number of units of the product ordered
  \item \textbf{order\_status}: indicating whether the order was \textit{Delivered to Buyer} or \textit{Returned to Seller}
\end{itemize}

\xhdr{Traditional Data Analysis} Jane uses a spreadsheet for her analysis (Fig.~\ref{fig:motivate}A). She explores the dataset in her spreadsheet tool. After grasping its structure, she zeros in on the task. She uses the spreadsheet's interface to filter the \textbf{order\_date} column for the month of November and the \textbf{order\_status} column for \textit{Delivered to Buyer}. She sees that there are two rows left, indicating two unique products were ordered in November and returned to the seller.  

In contrast, Kate opts to use computational notebooks for data analysis, employing Python code to investigate the analysis question (Fig.~\ref{fig:motivate}B). She writes code to read the dataset and to understand the data. 
She then writes code to filter the \textbf{order\_date} column for the month of November and the \textbf{order\_status} column for \textit{Delivered to Buyer}. In her workflow, Kate validates her operations by writing code to get a quick sense of the intermediate data produced. Like Jane, Kate arrives at the same conclusion. Throughout this process, Jane and Kate are actively engaged in the data and operations, giving them confidence in the correctness of their conclusion.

\xhdr{AI-Assisted Data Analysis}
Alex, meanwhile, decides to leverage an AI assistant for help. He uploads the dataset and writes a natural language prompt: \textit{How many items purchased within the month of November were returned to seller?}

The AI assistant writes and executes code to read the dataset. Next, it performs the analysis task, generating and running code before arriving at a final answer of 5. During this, the AI assistant also explains its steps in natural language. Because Alex was not directly involved in the analysis, he needs to validate its answer by inspecting the AI-generated output (Fig.~\ref{fig:motivate}C). He reads over the AI's natural language explanation of its procedure and skims the code briefly. Without fully understanding the code, he deems the answer to be correct. However, upon comparing his answer with Jane's and Kate's, Alex realizes the AI made a mistake. Looking through the intermediate data in Kate's work, Alex realizes the AI assistant calculated the number of units returned rather than the number of \textit{unique} products returned. 

The errors in AI-assisted data analysis are subtle and require the analyst to carefully scrutinize the AI's procedure and associated data involved. Additionally, current AI assistants do not facilitate the exploration of data along with the AI's code and natural language explanation, thereby constricting analysts' verification workflows. Further, it is unclear how analysts go about verification. Therefore, this paper seeks to understand analysts' workflows and identify opportunities for improvement.
% for analysts of various backgrounds and workflow tendencies.


==> 4-related-work.tex <==
\section{Background and Related Work}
% \tim{personally I prefer some intro sentence here}

\subsection{AI-Based Tools for Data Science Execution}
\label{sec:bg_automated}
% As writing data science code can be challenging and time-consuming, the community has developed a gamut of automated tools to help analysts in the process. Tools such as \textit{Mage}~\cite{Kery2020mageFM}, and \textit{Wrex}~\cite{Drosos2020WrexAU} provide users with graphical user interfaces to specify data wrangling code and associated manipulations. \textit{Glinda}~\cite{DeLine2021GlindaSD} uses a domain-specific declarative language for data science live programming. Meanwhile,~\textit{Mito}~\cite{diamondreivich2020mito} and \textit{B2}~\cite{Wu2020B2BC} enable users to directly interact with data using spreadsheet interfaces and dashboards, respectively, automatically generating the interaction's associated code. Despite simplifying the process, these tools target or were evaluated with data scientists with computation expertise. Users of \textit{Wrex} for example, commented how the availability of readable code allowed them to verify the transformation of the tool. What if the analyst was not able to understand the code? In this work, we explore how data analysts without programming expertise understand the processes of an AI-based analysis assistant. 

AI-based code assistants can enable analysts to conduct analyses as end-user programmers~\cite{Liu2023WhatIW, Ko2011TheSO}. With tools such as Github Copilot and ChatGPT, analysts' intent specified through natural language can be more expressive and approachable than those conveyed in domain-specific programming languages~\cite{DeLine2021GlindaSD, Gulwani2014NLyzeIP}. Given the potential of AI-supported natural language programming, there is a growing body of research in the value and usability of these tools~\cite{Sarkar2022WhatII, Liang2023UnderstandingTU, Vaithilingam2022ExpectationVE, Baker20161500SL, Dibia2022AligningOM, GitHubCopilotResearch}. These works focus on programmer experiences with AI-based code assistants and find common challenges in comprehending and verifying the AI-generated code~\cite{Liang2023UnderstandingTU, Vaithilingam2022ExpectationVE, Sarkar2022WhatII}. 
% In particular, Sarker et al.~\cite{Sarkar2022WhatII} noted the difficulty of code comprehension and verification as two central challenges in AI-assisted programming. 

Here, we build on prior work and study the verification challenges for data analysts as end-user programmers~\cite{Ko2011TheSO}. Compared to software engineering, data analysis is more exploratory and iterative~\cite{Kery2017ExploringEP, Pirolli2007TheSP, Liu2019PathsEP, Rule2018ExplorationAE} as code is not the deliverable but the outcome of the analysis~\cite{Epperson2022StrategiesFR, Kandel2012EnterpriseDA}. Importantly, making sense of the data is an integral part of data analysis~\cite{Pirolli2007TheSP, Russell1993TheCS, Grolemund2014ACI, Koesten2019TalkingDU}. While existing work has studied how programmers validate AI-written code for general programming tasks~\cite{Barke2022GroundedCH}, our work observes how data analysts' \textit{sensemaking} behaviors interplay with their verification of AI-generated analyses.
% Central to this data sensemaking process involves additional visualization artifacts~\cite{Grolemund2014ACI, Batch2018TheIV}.

AI-based analysis assistants have also received great attention. Prior work has explored the design of analytical chatbots~\cite{Zhi2020GameBotAV, Kassel2018VallettoAM, Hoon2019InterfacingCW} such as what should the responses be from such an assistant~\cite{Setlur2022HowDY} and how analysts can request, specify, and refine assistance~\cite{Mcnutt2023OnTD}. Given the attention and promise, these assistants have been integrated into popular analysis environments such as computational notebooks~\cite{PerryMallick2023, Gu2023HowDD} and spreadsheets~\cite{Stallbaumer2023}, and released as standalone systems~\cite{Dibia2023LIDAAT, Datagran2023}. In contrast, we examine these tools from the perspective of supporting analysts' understanding and verification of AI-generated analyses, especially as AI-assistants can specify sequences of data operations (e.g., Fig.~\ref{fig:motivate} right). In particular, we contribute the first user study examining the common behaviors and challenges in verification workflows.

\subsection{Understanding and \rr{Sensemaking} in Data Analysis}
\label{sec:bg_understand_analysis}
% Given the potential high stakes decisions based on data analysis findings, ensuring the validity of analyses is crucial.
Prior work has found that data scientists often compare conclusions with prior analyses and existing data~\cite{Kim2016TheER, Liu2019PathsEP}. Likewise, as part of data science collaboration and communication, it is common for data analysts to interpret and understand the results of another analyst's work~\cite{Zhang2020HowDD, Pang2022HowDD, Crisan2020PassingTD, Kim2018DataSI}. During this sensemaking, analysts often need help managing, tracking, and comparing the iterative and messy nature of their computations~\cite{Kery2019TowardsEF, Kery2018TheSI, Head2019ManagingMI, Wang2020AssessingAR}. To support this, prior work has explored how to help analysts track the data provenance in their analyses~\cite{Kery2019TowardsEF, Kery2017VarioliteSE, Wu2020B2BC} and visualize how their data changes throughout various data operations~\cite{Wang2019HowDS, Pu2021DatamationsAE, Xiong2022VisualizingTS}.


While existing research has focused on understanding human-written analyses, there are key differences between understanding analyses written by a human, and those written by an AI. People develop diverse perceptions and levels of trust in AI systems~\cite{Khadpe2020ConceptualMI, Jung2022GreatCO, Devito2018HowPF, Gu2023HowDD}, leading to distinct behaviors when evaluating AI-generated analyses. For example, McNutt et al.~\cite{Mcnutt2023OnTD} observed that some data scientists naturally trust analyses written by a colleague and may overlook code auditing. Additionally, social factors in data analysis communication often result in communicating asynchronously~\cite{Wang2019HowDS}, employing multiple platforms (i.e., Slack, Zoom, Google Docs etc.)~\cite{Pang2022HowDD}, and selectively sharing information~\cite{Pang2022HowDD, Liu2019PathsEP}. These qualities are less likely to appear when interacting with an AI-assistant.
Therefore, AI analysis assistants present a unique paradigm for analysis verification and sensemaking. Given the widespread deployment of AI-based tools, our work seeks to understand the intricacies of this paradigm. 
% Inspired by the designs in common data science tools, we build a design probe that provides analysts with a reasonable variety of artifacts and interactions to verify AI-generated outputs. Using our probe in a user study, we mimic a realistic verification experience, observe naturally occurring workflows, and elicit responses for preferred interactions. 

\subsection{Understanding and Verifying LLM Outputs}
\label{sec:bg_verify_ai}
% Prior work on AI explainability centered around decision-support scenarios, where the AI's prediction is limited to categorical variables~\cite{Adadi2018PeekingIT, Guidotti2018ASO, Linardatos2020ExplainableAA}. However, less is understood for generative AI, in which there can be multiple correct answers and each generation involves hundreds of individual token outputs~\cite{Vasconcelos2023GenerationPA}.

Prior work in the Human-Centered Explainable AI community has emphasized the goal that understanding AI revolves around empowering individuals to fulfill their objectives~\cite{Ehsan2021ExplainabilityPB, Liao2020QuestioningTA, Liao2021HumanCenteredEA, Kim2022HelpMH}. Following this perspective, recent work has explored ways to make LLMs more interpretable as they present their own explainability challenges~\cite{Sun2022InvestigatingEO, Vasconcelos2023GenerationPA, Dibia2022AligningOM}. Specifically, these works have explored opportunities for AI-code assistants in programming applications and proposed different explainable AI (XAI) features to guide the programmer's understanding of the model. In contrast, our work focuses on XAI features for data analysts. As data sensemaking is inherent in data analysis~\cite{Grolemund2014ACI, Koesten2019TalkingDU}, we explore specific features that help analysts in following the AI's data operations (e.g., via the natural language explanation and associated data tables).

We note that understanding and verifying AI-generated outputs can involve additional follow-up prompts to the AI assistant~\cite{Liu2023WhatIW, Lakkaraju2022RethinkingEA}. In this work, we focus on understanding the usage of supporting artifacts and disentangle the verification workflow using these artifacts from prompt writing (Sec.~\ref{sec:method_design}). Works studying abstraction matching~\cite{Liu2023WhatIW}, prompt writing~\cite{ZamfirescuPereira2023WhyJC}, and repair of AI-generated programs~\cite{Olausson2023DemystifyingGS, Ashktorab2019ResilientCR} are related but distinct.

% Therefore, we develop a prototype interface to probe analysts' workflows and conduct an empirical study with real datasets, and examples from state-of-the-art AI-based assistants. We contribute the first user study to explore the behaviors and challenges in verifying AI generations in the context of data analysis. 





% uncertainty highlighting of LLMs to programmers~\cite{Vasconcelos2023GenerationPA, Sun2022InvestigatingEO}.

% Sun et al.~\cite{Sun2022InvestigatingEO} proposed highlighting the probability that the model would generate a specific token




% Generation Probabilities Are Not Enough: Exploring the Effectiveness of Uncertainty Highlighting in AI-Powered Code Completions~\cite{Vasconcelos2023GenerationPA}

% Expectation vs. Experience: Evaluating the Usability of Code Generation Tools Powered by Large Language Models
% ~\cite{Vaithilingam2022ExpectationVE}  found that
% programmers found it challenging to read and debug suggestions from Copilot, particularly
% when its suggestions were long


% Effect of confidence and explanation on accuracy and trust calibration in AI-assisted decision making~\cite{Zhang2020EffectOC} "Previous research has shown that techniques such as communicating uncertainty"


% Does the Whole Exceed its Parts? The Effect of AI Explanations on Complementary Team Performance~\cite{Bansal2020DoesTW}


% How Can We Know When Language Models Know? On the Calibration of Language Models for Question Answering~\cite{Jiang2020HowCW}: traditional NLP for QA

% distinguish between NLP tasks

% verifying hallucination. quick sentence.

% in contrast to that work we are focusing on human in the loop

% not evaluating model’s performance

% difference between verifying facts and


% Investigating Explainability of Generative AI for Code through Scenario-based Design~\cite{Sun2022InvestigatingEO} insight into the explainability-related needs of programmers, and found that
% their design, which highlighted uncertainty in a line of code using a wavy line, revealed the
% need for: alternative outputs for uncertain code suggestions, explanations for why the AI was
% uncertain, and the ability to display different levels of uncertainty (e.g., using more colors
% or hues). 


% "However, programmers
% may incorrectly attribute the uncertainty as indicating a potential error. Likewise, if there
% are multiple correct ways to implement a function, they cannot all simultaneously have high
% generation probability, meaning that some will necessarily appear “uncertain.” The discon-
% nect between the meaning of a generation probability and a programmer’s intuition may be
% exacerbated by the fact that language models can be confidently wrong, producing fluently
% inadequate [ 37] outputs that are merely statistically plausible linguistically, but that lose or
% hallucinate information [e.g., 4, 25]."



% Is GitHub Copilot a Substitute for Human Pair-programming? An Empirical Study~\cite{Imai2022IsGC} "users may not trust generated
% code compared to code produced by a human pair programmer"

==> 5-method.tex <==
\section{Method: Design Probe and Prepared Tasks}
\label{sec:method}

In this work, we aim to study how analysts verify AI-generated analyses with features that support data sensemaking. In doing so, we wanted to minimize the impact of variations in the dataset, task difficultly, prompt expertise, and AI responses. 
To facilitate analysts' natural sensemaking workflows when working with data, we chose to purpose-build a design probe~\cite{boehner2007hci} and provide additional data artifacts based on recommendations from prior work~\cite{Alspaugh2019FutzingAM, Kery2019TowardsEF, Choi2023TowardsTR, Batch2018TheIV, Kery2018InteractionsFU, Wu2020B2BC, Moritz2017TrustBV}. We made this decision because existing assistants, such as Code Interpreter~\cite{openai_codeinterpreter}, do not allow easy exploration of data and only provide natural language explanations, code, and execution outputs. 
% % Our goal is not to evaluate our specific interface but rather to understand workflows that emerge when verification artifacts are available. 
% To reliably observe analysts' verification workflows and usage of verification artifacts, we deliberately restricted the scope of our study, aiming to minimize potential confounding factors. Specifically, as opposed to having analysts interact directly with an AI assistant, we chose the prompts, datasets, and AI-generated responses in our verification tasks a priori and prevented follow-up prompts.
In this section, we discuss the key design considerations involved in our study (Sec.~\ref{sec:method_design}) before outlining the specific design of our probe (Sec.~\ref{sec:method_probe}) and the preparation of our study tasks (Sec.~\ref{sec:method_materials}).


\subsection{Design Considerations}
\label{sec:method_design}
In building our design probe and formulating our user study, we identified three central design considerations that involved different trade-offs outlined below. These decisions are guided by our goal to make reliable observations on analysts' \emph{verification workflows} with different \emph{supporting artifacts}, while minimizing distractions from other aspects of the data analysis workflow.
 
\xhdr{Using familiar and approachable supporting artifacts} 
A crucial decision in implementing our design probe revolved around the choice of data artifacts. One option is to incorporate customized feature-rich artifacts (e.g., those in \textit{Datamations} or \textit{DITL}~\cite{Wang2022DiffIT, Pu2021DatamationsAE}) and verification interfaces (e.g., incorporating visualization tools like \textit{Voyager}~\cite{Wongsuphasawat2016VoyagerEA, Wongsuphasawat2017Voyager2A} or \textit{PygWalker}~\cite{kanaries_pygwalker} for verificaiton). Alternatively, we could opt for integrating a core set of simpler, more user-friendly, and approachable data artifacts. These two options contrast with each other in terms of \emph{the richness of actions analysts can achieve with the interface} and \emph{the time and effort analysts need to spend to learn to perform these actions}. 
% However, this choice comes with the trade-off of complicating the tool and introducing steep learning curves~\cite{Grammel2010HowIV, Kwon2011VisualAR, Lee2016HowDP}. As result, such tools may not be obvious to all users and actually impede their verification workflows. On the contrary, we could opt for integrating a core set of standard, more user-friendly data artifacts but potentially constrain the long tail of analysts' actions. 

Ultimately, we opted for familiar and approachable artifacts as our study focus is to observe verification workflows: we determined that the challenges tied to learning and interpreting customized visual elements would limit our ability to observe these workflows~\cite{Grammel2010HowIV, Kwon2011VisualAR, Lee2016HowDP}. Likewise, while generic artifacts and interfaces may overlook some features experienced analysts could leverage, they let us focus on analyzing analysts' workflows across a broad audience and still gather concrete feedback on the features they want.


\xhdr{Focus on one turn of the human-AI interaction} 
Another choice that shaped our probe and study was whether or not to allow follow-up prompts to the AI as part of the verification workflow. On one hand, choosing to allow follow-up prompts enables analysts to use them in their verification. However, besides interpreting the AI's current output, analysts would need to grapple with the challenge of formulating prompts~\cite{ZamfirescuPereira2023WhyJC, Mishra2022HELPMT}. On the other hand, opting against follow-up prompts mitigates the impact of prompt expertise but at the cost of confining analysts' actions. In our study, we chose to zoom in on one turn of the human-AI interaction and disallow follow-up prompts. As every new prompt triggers a corresponding response from the AI assistant, continuous interpretation and verification of AI-generated outputs are inevitable. In reducing the scope, we chose to thoroughly observe how analysts understand the AI's outputs and interact with supporting artifacts. Similarly, aiding analysts in understanding the AI-generated output through artifacts  not only helps them rectify errors in immediate interactions but also craft more effective prompts in future engagements.


 % Our study is a first step in characterizing the verification workflows of AI-generated analyses.
\interfaceFig 


\xhdr{Prepare standardized task materials} The choice of datasets and verification tasks was also important to consider. One option is to allow analysts to work with their own datasets while interacting with the AI in real-time to verify the AI's outputs. Alternatively, we could pre-prepare the natural language prompts, associated datasets, and AI-generated responses. These choices underscore a trade-off between matching analysts' natural workflows and mitigating variability associated with generative AI and dataset complexity. In our study, to control potential confounding factors, we chose to prepare all task materials. Although this approach may differ from the scenario where analysts' verify their own datasets and analyses, it closely aligns with situations where analysts need to familiarize themselves with another analyst's analysis~\cite{Pang2022HowDD, Zhang2020HowDD, Koesten2019CollaborativePW}. To mitigate concerns related to dataset unfamiliarity, we carefully prepared approachable and realistic datasets from diverse domains, used prompts written by real-world data scientists, and provided additional background descriptions of the dataset and analysis motivation (Sec.~\ref{sec:method_materials}). Given our chosen approach, it would be interesting to apply the lessons learned in this study to analysts working on their own datasets and tasks (Sec.~\ref{sec:limitation}).


% While this mirrors analysts' natural workflows, it poses challenges in generalizing observations across analysts due to the lack of control over prompts, specific AI outputs, types and frequency of errors observed, and the datasets.  This approach reduces variability linked to generative AI and dataset difficulty but adds the drawbacks of introducing unfamiliar datasets and analyses along with prompts not crafted by analysts. However, this setting closely aligns with situations where analysts need to familiarize themselves with another analyst's analysis~\cite{Pang2022HowDD, Zhang2020HowDD, Koesten2019CollaborativePW}.


% Our design probe aimed to equip analysts with the essential tools such that their main focus remained on the verification of AI-generated analyses and not on prompt design. This allows us to control for the types of errors analysts encounter, the dataset scenarios, and prompting abilities of the analyst. 


% \begin{enumerate}
% \item \textit{DC 1 - Interactions should support data sensemaking activities.} Data analysts need to \textit{inspect} the data (i.e., the data quality, format, columns, values etc.) and \textit{engage} with the data (e.g., understanding relationships between columns, looking for outliers etc.) as part of data sensemaking activities~\cite{Koesten2019TalkingDU}. Prior work has detailed the importance of contextualized intermediate data visualizations for analysis provenance~\cite{Alspaugh2019FutzingAM, Kery2019TowardsEF, Choi2023TowardsTR, Batch2018TheIV, Kery2018InteractionsFU, Wu2020B2BC, Moritz2017TrustBV}. Notably, these works highlight the need for smooth transitions between the code and the data~\cite{Choi2023TowardsTR, Wu2020B2BC} and the underscore data tables~\cite{Batch2018TheIV} as an integral visualization component. Consequently, the tool should offer an interface and interactions that facilitate the visualization of data that is connected to the underlying code. 

% \end{enumerate}



% \subsection{Designing the Probe}
% Based this objective, we identify two design goals and comment on their tradeoffs.
% % that allow you study data analysts. \tim{based on what? where do they come from? }
% % \tim{bit subtle: are these design goals to support data analysts or are they properties your probe needs to satisfy in order to elicit realistic workflows that allow you study data analysts doing this... The writing jumps slightly between them. }
% \begin{enumerate}
%     % \item \textit{DG 1 - Enable end-user programmers.}
%     % We want the presentation of the AI's process and output to be comprehensible to end-users of varying programming expertise. As a result, it is insufficient to just present the code generated by the AI. 
    
%     \item \textit{DG 1 - Interactions should support data sensemaking activities.} Data analysts need to \textit{inspect} the data (i.e., the data quality, format, columns, values etc.) and \textit{engage} with the data (e.g., understanding relationships between columns, looking for outliers etc.) as part of data sensemaking activities~\cite{Koesten2019TalkingDU}. Prior work has detailed the importance of contextualized intermediate data visualizations for analysis provenance~\cite{Alspaugh2019FutzingAM, Kery2019TowardsEF, Choi2023TowardsTR, Batch2018TheIV, Kery2018InteractionsFU, Wu2020B2BC, Moritz2017TrustBV}. Notably, these works highlight the need for smooth transitions between the code and the data~\cite{Choi2023TowardsTR, Wu2020B2BC} and the underscore data tables~\cite{Batch2018TheIV} as an integral visualization component.
%     Consequently, the tool should offer an interface and interactions that facilitate the visualization of data that is connected to the underlying code. 

%     \item \textit{DG 2 - Approachable to analysts from different tool backgrounds.} The main goal of our probe is to understand analysts' processes. Because we are interested in analysts of various backgrounds, we want the tool to be approachable to a large audience. While certain features may benefit certain analysts, incorporating all features from existing data science tools could make the tool more complex and impede the actual verification process. With this in mind, the tool should include a range of artifacts commonly familiar to analysts, fostering natural verification workflows without a steep learning curve.
%     % \item \tim{rough transition on sentences 0 sounds like DG3 is really: allow analysts with a range of statistical and programming backgrounds to verify.... /} 

% \end{enumerate}
% These design goals inform our decisions around the user interface and associated interactions. 

\subsection{Design of the Probe}
\label{sec:method_probe}
Data analysts need to \textit{inspect} the data (i.e., the data quality, format, columns, values etc.) and \textit{engage} with the data (e.g., understanding relationships between columns, looking for outliers etc.) as part of data sensemaking activities~\cite{Koesten2019TalkingDU}. Therefore, we designed our probe with facilities for understanding the data. This includes data tables, and summaries and histograms of all the fields in the data. To support sensemaking while making components approachable, our probe incorporates abstractions of modalities found in popular data science tools: the code, code comments, natural language explanations, data tables, and visualizations~\cite{jupyterlab, tableau, rstudio, Drosos2020WrexAU, Kery2020mageFM, diamondreivich2020mito, Wu2020B2BC}. 

\xhdr{User Interface}
The probe's interface follows a multi-panel design. The main panel shows the chat interface between the user and the assistant (Fig.~\ref{fig:interface} left). The user's prompt and subsequent response from the assistant are shown. In the assistant's response, following Code Interpreter~\cite{openai_codeinterpreter} and explanation practices recommended and found favorable in prior work~\cite{Lakkaraju2022RethinkingEA, Sun2022InvestigatingEO, Drosos2020WrexAU}, the interface shows the assistant's natural language explanation of its procedure, associated code, code comments, and execution outputs (Fig.~\ref{fig:interface}A and B). These are interleaved together such that all artifacts are available at any time. In addition, because understanding the sequence of data manipulations is vital to understanding the output~\cite{Pu2021DatamationsAE, Xiong2022VisualizingTS},  the probe includes descriptions of any intermediate data computed as a result of an atomic data wrangling operation (Fig.~\ref{fig:interface}C)~\cite{Xiong2022VisualizingTS, Kasica2020TableSA}.

 Inspired by prior work detailing the importance of contextualized intermediate data artifacts for analysis provenance~\cite{Alspaugh2019FutzingAM, Kery2019TowardsEF, Choi2023TowardsTR, Batch2018TheIV, Kery2018InteractionsFU, Wu2020B2BC, Moritz2017TrustBV}, the probe includes a side data panel (Fig.~\ref{fig:interface} right) that allows analysts to view all relevant data in the AI-generated analysis. Having this as a side panel is helpful as it suggests the information is of global scope~\cite{Mcnutt2023OnTD}. Additionally, by keeping the data separate from the AI-generated analysis, the probe minimizes any interference to analysts following the AI's procedure in the main panel. In the side panel, data tables are shown (i.e., the original data and the results of intermediate calculations) as collapsible panels. Each collapsible panel includes a raw data table and a summary visualization of the table from ~\cite{observablehq_summary_table}. The summary visualization offers a quick visual summary of the overall table, the values and distribution of each column, and basic descriptive statistics.

\xhdr{User Interactions}
In the main panel, the probe's interactions prioritize easy access to the full/high-level abstraction of the procedure conveyed through the AI's natural language explanation. Because code and table descriptions can obstruct and interrupt this view, the code and intermediate data descriptions in the main panel are initially hidden which users can reveal via a show/hide button. Analysts can also access the side data panels within the flow of the AI's explanation via in-context buttons which open and close the corresponding panel (Fig.~\ref{fig:interface}E1 and E2).

In the side panel, analysts can perform basic operations on each table such as sorting columns and filtering rows based on specific values in the column(s). To support easy navigation between the data tables and AI's procedure in the main panel~\cite{Choi2023TowardsTR, Wu2020B2BC}, clicking on a data table scrolls the main panel to the corresponding context of that data table. 

\tableTasks

\subsection{Preparation of Study Tasks}
\label{sec:method_materials}
To prepare realistic analysis verification tasks and AI-written errors representative of those made by state-of-the-art AI assistants, we used the ARCADE benchmark dataset from Yin et al.~\cite{Yin2022NaturalLT}. ARCADE features multiple rounds of natural language intent to code problems (i.e. a natural language query, dataset, and code solution) situated in computational notebooks\footnote{these notebooks used datasets uploaded to \href{https://www.kaggle.com}{Kaggle} and encompassed data wrangling and EDA operations} written by data scientist annotators. In our task preparation, we ran queries from ARCADE on Code Interpreter~\cite{openai_codeinterpreter} and carefully selected a subset of queries that contained errors, had good coverage across a range of domains and error types, and were approachable to analysts (details in the appendix). These queries and Code Interpreter responses formed the backbone of our tasks. 

 In total, we prepared one tutorial task and 10 main tasks, 2 of which did not contain any errors, spanning 9 unique datasets (Table~\ref{tab:tasks}). For each task, we used the generated code from Code Interpreter's output to prepare intermediate data tables and table summary visualizations. To provide analysts with sufficient information, we prepared additional intermediate data tables for all major transformations, often breaking up chained function calls in the code. We then verified with multiple expert data scientists that these intermediate data tables were sufficient for the task. To ease dataset understanding and help participants focus on verification, we reduced the number of columns for excessively complex datasets. We made sure to leave enough extra columns irrelevant to the immediate analysis query such that the task remains non-trivial. In addition, we provided a clear ground truth motivation and a more detailed description of the analysis query. In the rest of the paper, to differentiate the two, we refer to the detailed description of the analysis query as the \textit{analysis goal}. Finally, we
provided a description of the dataset and what each column in the dataset represented.

In summary, we compiled the following primary materials for each task: the natural language query from ARCADE, the unmodified code, code comments, and natural language explanation response from Code Interpreter, the prepared data tables and visualizations (Fig.~\ref{fig:interface} right), and a detailed description of the motivation, analysis goal, and dataset.  




% We focus on end-user programmers. 
% We mimic the outputs of the Code Interpreter. 

% We show intermediary outputs as this has been said to be important in prior literature.
% Enable sort, filter etc.
% Intermediary data

% Summary visualization capturing the dataset. 





==> 6-study.tex <==
\tableParticipants

\section{User Study}
\label{sec:study}

Using our probe and prepared tasks, we conducted a user study to observe analysts' verification workflows of AI-generated analyses. Our goal was not to evaluate our specific interface but rather to understand behaviors that emerge when verification artifacts are available. Three research questions guide our study design and analysis. 
\begin{itemize}
    \item \textbf{RQ1 - Behaviors:} \rr{\rqWorkflows}
    \item \textbf{RQ2 - Artifacts:} \rr{\rqArtifacts}
    \item \textbf{RQ3 - Background:} \rr{\rqBackground}
\end{itemize}

% A central study design decision was to prepare examples of errors and AI outputs a priori as opposed to having analysts interact directly with an AI assistant. This was motivated by a couple of reasons. First, by removing the variability of generative AI, we controlled for a consistent experience across participants, ensuring they all faced the same AI-generated mistakes. Second, we disentangled the process of crafting prompts for the AI (both initial and follow-up) from the process of comprehending the AI-generated outputs. Our design probe aimed to equip analysts with the essential tools such that their main focus remained on the verification of AI-generated analyses and not on prompt design. 

% \ken{TODO: include somewhere that the reason we are not using live examples. We choose to do static to avoid the pitfalls of: ---. Clearly indicate why static is better}


\xhdr{Participants}
We recruited participants from a large data-driven software company and advertised an opportunity to work with AI-generated analyses. Participants were recruited via email based on data analysis interest groups and organization mailing lists. We selected participants with data analysis experience and from diverse backgrounds, including how often they performed data analysis, the types of tools they used for analysis, and their self-reported comfort with programming (Table~\ref{tab:participants}). Participants were compensated with a \$30 USD Amex gift certificate. 


% \xhdr{Materials}
%  In preparation for our study, we wanted to find realistic analysis verification tasks and AI-written errors representative of those made by state-of-the-art AI assistants. To do so, we used the ARCADE benchmark dataset from Yin et al.~\cite{Yin2022NaturalLT} which features multiple rounds of natural language intent to code problems (i.e. a natural language query, dataset, and code solution) in computational notebooks written by data scientist annotators. These notebooks used datasets uploaded to Kaggle\footnote{https://www.kaggle.com}, a popular online community for data scientists, and encompass data wrangling and EDA tasks. To avoid datasets overlapping with the training data of LLMs~\cite{OpenAI2023GPT4TR, Brown2020LanguageMA}, we chose natural language queries associated with datasets uploaded to Kaggle after February 2022. This included 660 queries from 70 distinct datasets.

% We selected a subset of analysis queries that were incorrectly answered by current state-of-the-art LLMs (GPT-4 and Code Interpreter). First, we tested the 660 queries against GPT-4~\cite{OpenAI2023GPT4TR} using its API (temperature=0.7, n=3). For this, GPT-4 was provided a dataset summary (example in the Appendix) similar to that of other LLM-based analysis tools~\cite{Dibia2023LIDAAT}, a scaffold to write code in, and the natural language query. Next, we sampled a set of 50 queries that resulted in incorrect outputs from GPT-4, specifically selecting more complex queries with a high number of Pandas API calls in the solution. These queries (and corresponding datasets) were then presented to Code Interpreter. Code Interpreter executed the code for the analysis, and detailed its steps in natural language. 

% After manually inspecting the 50 queries GPT-4 struggled with, we identified 22 that were also incorrectly answered by Code Interpreter. These errors included bad calculations, semantic misinterpretations of the prompt, and misunderstandings of the data. We then chose a subset of these 22 queries that cover a variety of error types (i.e., misunderstanding column semantics, bad calculations, or misunderstanding the query) and involve datasets and domains that were approachable to general audiences. Using this subset, we constructed the tutorial and primary tasks of our study. Sometimes, Code Interpreter encountered ambiguities and sought clarification from the user. For these cases, we included a follow-up prompt and integrated the multi-turn interaction into our study tasks. In total, we prepared one tutorial task and 10 main tasks, 2 of which did not contain any errors, spanning 9 unique datasets (Table~\ref{tab:tasks}).

% For each task in our study, we prepared intermediate data tables and table summary visualizations for each code snippet in Code Interpreter's analysis. To provide analysts with sufficient information, we prepared additional intermediate data tables for all major transformations, often breaking up chained function calls in the code. We then verified with multiple expert data scientists that these intermediate data tables were sufficient for the task. To ease dataset understanding and help participants focus on the verification process, we reduced the number of columns for excessively complex datasets. We made sure to leave enough extra columns irrelevant to the immediate analysis query such that the task remains non-trivial. In addition, we provided a clear ground truth motivation and a more detailed description of the analysis query. In the rest of the paper, to differentiate the two, we refer to the detailed description of the analysis query as the \textit{analysis goal}. Finally, we
% provided a description of the dataset and what each column in the dataset represented.

% To summarize, we compiled the following primary materials for each task: the natural language query from ARCADE~\cite{Yin2022NaturalLT}, the code, code comments, and natural language explanation response from Code Interpreter~\cite{openai_codeinterpreter}, the data tables and visualizations we prepared (Fig.~\ref{fig:interface} right), and a detailed description of the motivation, analysis goal, and dataset.  
% \tim{refer to fig 2 as illustrating example}

\xhdr{Study Procedure}
We conducted our study remotely with participants sharing their screens over a video conferencing tool. Because our design probe was built as a web application, participants loaded the interface on their computer with their choice of browser. 

The study was structured into three parts lasting approximately 60 minutes total: a tutorial phase ($\sim$10 min), an activity phase ($\sim$40 minutes) in which participants worked through the prepared tasks, and a semi-structured interview phase ($\sim$10 minutes). In the tutorial phase, we presented participants with the following scenario: \textit{Imagine having an intern who is provided with a dataset to address an analysis problem. The enthusiastic intern decides to use an AI assistant to complete the problem, correctly uploading the relevant dataset and crafting a prompt that is their interpretation of the original analysis problem. The AI assistant produces an output but the intern is unsure whether it is correct.}

We clarified that the input to the AI assistant is only the intern's prompt and the uploaded dataset. In particular, we directed analysts not to focus on the quality of the prompt, but on the AI-generated output in response to the prompt. We mention that although the code executes, there might be issues with the information the AI uses or how it interprets the intern's prompt. Next, we presented the participants with the intern's prompt and the assistant's response in our interface (Fig.~\ref{fig:interface}). We asked participants to determine if the AI assistant's answer correctly addressed the initial problem, and if not, point to reasons why they think there was a mistake. To eliminate the challenge of participants having to craft their own prompts—a task that presents its own set of difficulties~\cite{ZamfirescuPereira2023WhyJC}—we chose to assign the responsibility of prompt authoring to the intern. This choice also dissociated participants' personal preferences for how they would write prompts which is not the core focus of our study. 
% \tim{didn't get there yet but helping analysts write good prompts could be called out as a need again in discussion}

After introducing the analysis scenario, we gave participants a brief walk-through of the interface (Fig.~\ref{fig:interface}). We then had participants complete a fixed tutorial task to familiarize themselves with the interface (T0 in Table~\ref{tab:tasks}). The task intentionally contained an error in which the AI assistant misinterpreted the values of a column and poorly sorted the answer. This strategy aimed to make participants cognizant of potential assistant errors and to encourage vigilance in subsequent tasks. 
% \tim{nice!}

Next, in the activity phase, participants read the analysis goal and reviewed the work of the assistant and intern. We assigned tasks to participants to ensure that, collectively, all tasks were covered (Table~\ref{tab:tasks}). For all tasks in the study, the motivation, analysis goal, and description of the dataset were always available in a left side panel (see appendix for an example). To make sure the participants fully understood the analysis goal, we discussed any areas they found unclear. We also clarified any questions about the dataset or analysis goal while participants were working through the task. To reduce time pressure and encourage a realistic workflow, we emphasized the exploratory nature of our study, allowing participants to work at their own pace until they were satisfied with their conclusion. After completing each task, participants were asked to complete a brief survey that asked for a confirmation as to whether the AI's generation was erroneous % \tim{it might not be clear this is the numerical?! answer to the original question. note that if you use answer here I think question makes sense earlier. or query/result? } 
and their reasoning.

While participants were completing the tasks, we encouraged them to think aloud and describe their reasons for interacting with different components of the interface. If they remained relatively silent, we  regularly prompted them to speak about their workflow. We provided minimal help beyond clarifying the analysis goal or semantics of the data. Finally, in the semi-structured interview, we asked open-ended questions to understand participants' backgrounds and prior experiences, overall verification workflows, and rationales behind their behaviors.

\tableDefs

\xhdr{Transcript and Workflow Analysis}
% With consent from participants, we recorded the participants' audio and screens during the study. One author was sitting in the study and recorded notes throughout. Using the recordings, notes, and audio transcripts two authors identified all interactions and observations related to participants' verification process and anything that might inform their behavior. 
To identify recurring themes, two authors reviewed the participants' screen recordings,  engaged in several rounds of open coding, and had multiple meetings to refine their observations. The themes we observed highlighted variations in participants' workflows and the artifacts they used. In the analysis and results, we distinguish between \textit{data artifacts} (those in Fig.~\ref{fig:interface} right) and \textit{procedure artifacts}~(those in Fig.~\ref{fig:interface} left). Data artifacts pertain to the original, intermediate, and result data (i.e., the data table and summary visualization). Conversely, procedure artifacts encompass the natural language explanation, code/comments, and the AI's explanation and interpretation of its result.

Additionally, to systematically understand participants' verification workflows, we delineated these into sequences of primary observations. 
Informed by the themes from open coding, the two authors who developed the themes drafted an initial set of observation labels (e.g., \textit{read data table} or \textit{raising a consideration}). Both authors annotated a few participants' workflows independently before meeting to resolve ambiguities and unclear interpretations. These discussions facilitated a refinement of the observation labels by broadening their scope. Using the final refined set of labels~(Table~\ref{tab:labeldefs}), they rewatched the recordings and annotated all end-to-end verification workflows in the study (see Fig.~\ref{fig:cases} for examples), including observations of the artifacts being used. 

Each workflow starts when participants began verifying the AI-generated analysis (after understanding the task and data) and ends when they confirmed or rejected the existence of an error. We list all participants' verification workflows in the appendix.  

% Our findings highlight common workflow patterns and how different artifacts supported these workflows. 









% reveal high level patterns of activities. \tim{did not understand this step}  \tim{do you describe these labels/categories somewhere. at least in appendix with definitions or so?}








==> 7-results-submission.tex <==
\casesFig

\section{Results}
\label{sec:results}

% \ken{Branching \cite{Jiang2023GraphologueEL, Suh2023SensecapeEM}}

Participants engaged in a variety of different steps to identify potential issues and ultimately confirm or reject the AI's analysis. Our user study uncovered two common high-level workflows analysts used within their verification processes:~\textit{procedure-oriented workflows} and \textit{data-oriented workflows}~(Fig.~\ref{fig:workflows}) (\textbf{RQ1}).

Within a verification process, participants adopting a \processworkflow~were primarily focused on validating the AI's procedure, possibly drawing upon data artifacts to aid their understanding. In contrast, participants following a \dataworkflow~gave precedence to scrutinizing the data involved in the analysis, relegating the AI's procedure to a supplementary role. The distinction between these workflows lies in the participants' intention. Participants following procedure-oriented workflows were concerned with \textit{what does the AI do?} Meanwhile participants following data-oriented workflows focused on \textit{does the data make sense?} This was clear from observing their interaction patterns and verbal comments. For example, while some participants engaged extensively with intermediate datasets, their main goal in those moments was to confirm the correctness of the AI's procedure; these behavioral patterns were labeled as procedure-oriented workflows with the use of data artifacts as secondary support (i.e., \process~).

Furthermore, participants frequently shifted workflows before and after they noticed an issue in the AI's analysis (see Fig.~\ref{fig:cases} for examples). Participants usually followed a \processworkflow~initially during their verification process. Upon identifying a concern, their strategies diversified, delving deeper to explore and validate the perceived issue~(Table~\ref{tab:freq-of-workflows}). In undertaking these workflows, analysts leveraged both data and procedural artifacts, not only as central elements in their primary workflow but also as supporting artifacts to both reinforce their comprehension and validation of  the primary workflow~(Fig.~\ref{fig:artifacts}) (\textbf{RQ2}). From our post-task interviews, we observed how analysts' backgrounds influenced them towards ~\dataworkflows~or \processworkflows~and how a familiarity with data operations and basic programming helped them understand the AI's procedure (\textbf{RQ3}). 

In this section, we describe procedure-oriented (Sec.~\ref{sec:results_pworkflow}) and data-oriented (Sec.~\ref{sec:results_dworkflow}) workflows; the focal points within these workflows, the artifacts used (both as the main focus and secondary support) and how these workflows led analysts to identify issues. Subsequently, we outline observations related to analysts' backgrounds and how this informed their verification processes (Sec.~\ref{sec:results_bg}).


\subsection{Procedure-Oriented Workflows}
\label{sec:results_pworkflow}

We observed most participants (18/22) followed all or parts of the AI's procedure at some point during their verification processes (44/52). Participants focused on different aspects of the procedure and often leveraged data to support their understanding and validation of information from the procedure. 


\workflowsFig
\tableWorkflows
\subsubsection{Focal Points in Procedure-Oriented Workflows}
% Process - High-level steps
In \processworkflows~, participants focused on different facets of the AI's analytical procedure utilizing all procedure artifacts in support. Some participants looked over the AI's procedure to get a high-level understanding of its analysis steps (P1, P2, P4, P8, P11, P17, P18, P20). For instance, in T9, P18 wanted to understand how the AI arrived at a particular actor-director pair in the result: \shortquote{I'm trying to read the code and I'm trying to understand ... like how is it generating that pair and if there is any error in that process.} In some cases, participants gained confidence in the AI's correctness
% \steve{I noticed this in many places, you should probably nearly always use an article in front of AI - the AI's correctness - in this case, but many times you don't} 
from this high-level understanding  (P1, P2, P11, P20). For example, P1 confirmed their understanding after reading the AI's  procedure one last time:\shortquote{seems reasonable to me.} P11 was reassured by the AI's overall procedure matching their own: \shortquote{the steps it described is exactly what I would have done but in SQL.} In other cases, participants' focus on the procedure helped them notice and subsequently confirm a particular step the AI did wrong (P4, P8). For example, P4 and P8 both noticed from the NL explanation that the AI's order of analysis steps were incorrect [T5]. In T6, similar to P11, P4  broke down the general steps on their own and realized the AI missed calculating the average after inspecting the AI's procedure.  

In addition, participants focused on lower-level details involved in the AI's data operations  (P2, P7, P8, P9, P10, P11, P13, P15, P17, P22). Participants checked functions used in the code, logic around the data operations, and specific result values. P13 was especially vigilant making sure that \shortquote{the spelling was correct} in the data columns mentioned in the code, and that \shortquote{syntactically ... (they) appear to be correct.} P19 was also following the AI's data operations to see how it handled unusual values in the dataset the AI had identified earlier in its procedure. Focusing on low-level details was one way participants gained confidence in the AI or noticed issues (P7, P8, P10, P11). For instance, in T9, P10 focused on the AI's data operations in the code which they attributed to helping them conclude the AI had indeed found the highest count. P11, while not the most comfortable with Python, used code comments to translate the AI's procedure into familiar data operations, noticing the AI's procedure was inconsistent with the analysis goal description [T8].

Moreover, participants focused on the AI's Natural Language (NL) explanation of its result and found discrepancies by comparing this against their common knowledge. For example, P10 felt that \shortquote{2800 flights felt like a lot} for a day [T5], leading them to investigate the AI's procedure. Similarly, from inspecting the AI's explanation of the result, P6 noticed \shortquote{Jurassic World is not a Bollywood movie} [T4]. These discrepancies prompted them to question the AI's data operations and understanding of the dataset . 

Within \processworkflows~participants were also keen on verifying the consistency in the AI's procedure, that the NL explanation outlining its high-level analysis steps matched the code detailing the specific data operations (P5, P11, P17, P22). Finally, participants used the AI's procedure to verify its interpretation of the prompt and original dataset (P4, P12). For instance, for T7, both P4 and P12 noticed discrepancies in the AI's understanding of the data from its NL explanation stating an incorrect interpretation of a column.
% \ken{Could we say: The process also enabled participants to identify a lack of specificity in the prompt. While prompt-writing was not the focus of our study, we discuss how prompt specification and how verification processes fit in Section~\ref{sec:discussion_prompt}}

\artifactsFig

\subsubsection{Data Artifacts in Support of Validating the Procedure}
\label{sec:results_data_support_procedure}

We found data artifacts were often indispensable during participants' \processworkflows~(17/22 participants and 41/52 verification processes). 
% This included participants quickly inspecting the data associated with the the AI's procedure or replicating the AI's data operations to support their verification of the AI's procedure. 

Some participants glanced at the data artifacts to check things they noticed in the AI's procedure (P6, P8, P22). For instance, P22 noticed that the AI's calculation for the average price of gourmet food was not a number, prompting them to check the original data table and discovering that the AI used the wrong column name [T2]. Similarly, participants used data artifacts to conduct data sanity checks to verify the procedure (P1, P3, P4, P19, P21, P22). For instance, P19 wanted to see if percentages in a column added up to 100: \shortquote{If the percentages tied to 100\%, I would feel confident just at a glance that you know everything and action was allocated to one of those languages} [T8]. 

In other cases, participants tried to replicate the AI's data operations using the supported functionalities in the data tables to compare with the result in the AI's procedure and verify what the AI did (P2, P9, P12, P14, P22). Consequently, participants often noticed discrepancies between the AI-generated outputs and their calculated results. As an illustrative example, in T6, P14 used the data tables throughout their verification process to manually follow the AI's procedure and confirm that the AI made a mistake when the result did not align with their manual calculations [T6]. In an another example, P22 filtered on the \textit{frequency} column following the AI's steps to see how many rows were filtered out [T10]. From these observations, we observed  participants both relied on simple checks and detailed calculations on the data artifacts to verify the procedure.

% ========= Data Oriented Workflows ========

\subsection{Data-Oriented Workflows}
\label{sec:results_dworkflow}
Data-oriented workflows primarily focused on validating and understanding the data, occasionally using the AI's procedure to make sense of things noticed in the data. This workflow was commonly observed in participants after they had identified a potential issue, a trigger that spurred them to investigate the data (Table~\ref{tab:freq-of-workflows}). Overall, we observed 18/22 participants in 25/52 verification processes adopting data-oriented workflows. Likewise, 15 participants in 17 verification processes included data-oriented workflows in response to noticing an issue.

\subsubsection{Focal Points in Data-Oriented Workflows} 
\label{sec:results_focal_in_data}
Participants in \dataworkflows~focused on the data in a variety of ways. Some participants (P3, P7, P15, P19) were keen on understanding the data (original and intermediate) and the specific columns relationships that were pertinent to the analysis goal. For instance, P7 adopted a \dataworkflow~ using only data tables at the beginning of their process, identifying a data quality issue in the frequency column while exploring the column of interest in the analysis goal [T10]. Meanwhile, for P9, a prototypical data-oriented participant, their \dataworkflow~involved comparing all data tables [T9]. Specifically, they delved into the directors and actors intermediate data tables to gather an expectation of what they would expect in the subsequent merged data table (Fig.~\ref{fig:workflows} third row). After, they checked if specific actors in the result data existed in the merged data. In the process, they spent significant time forming an expectation of the result data, transitioning back and forth between all data tables. Upon perceiving a discrepancy between the number of rows in the merged data table and their expectations of the count from a quick mental calculation, they became skeptical of the AI-generated output. In contrast, P17 simply used the intermediate data tables to quickly compute the data operations for the analysis goal on their own: \shortquote{intermediate code is less useful ... I would go here (intermediate data table) and then do a sort on it myself.} While this might have been doable in the context of the datasets and tasks in our study, it might not be as easy with more AI-generated analyses involving complex operations or large datasets.

% P19 gain confidence on columns of data by trying to arrive an answer by myself based on a straightforward dataset. [Movie Content]

% \tim{interesting, I imagine you can't do that at some scale/complexity any more or as easily?}

Through closely examining the data tables, participants were able to identify issues with the AI-generated analyses (P1, P3, P7, P9, P13, P15, P16). For instance, from the original data table, P1 noticed that there were also the \textit{Nivea Men} brand in the dataset which the AI missed (Fig.~\ref{fig:cases} first row), ultimately leading them to confirm that the AI-generated analysis contained an error. In other cases, participants went into \dataworkflows~ after noticing an issue. Participants often went into the data tables for further verification on the exact data. While some participants (P2, P15, P16, P20, P22) identified the source of the issue through eyeballing  different data tables, others followed a ~\dataworkflow~to check more closely the potential source of an issue (P4, P5). In T2, P5 correctly noticed that there was no consideration for \textit{Nivea Men}. To explore this further, they focused on the original data table, filtering for rows in which the brand was \textit{Nivea} and applying additional filters to spot check specific products [T2]. Similarly, to affirm their suspicions of an error, P4 investigated the final result table after noticing the AI may not have grouped rows by \textit{flight code} (Fig.~\ref{fig:cases} second row) [T5]. 

% For example, P2 used the data summary to spot if anything was unexpected, stating, \longquote{I do like the summary thing because I did end up looking at that to see if like what the data types were and like what categories were and if something sticking out there that I didn't expect.} 
% Similarly, in T5,  P4 investigated the result table, concluding that it was not sorted by flight code [T5]. %P15 was surprised to see a Hollywood movie in the result table of the Bollywood dataset. P16 noticed that a hotel with a 0 ranking was never in the 2021 ranking in the Hotels dataset. P22 noticed that the intermediate table in the Movie Content dataset was inverted, with the wrong axis. For instance, P2, during the Hotels task, did not bother looking at the code and the intermediate tables. They jumped to the conclusion that the AI's output was incorrect based on how the data was presented with bad column names. Directly from the result data table, P20 noticed the unique SKUs were not quantity and confirmed that the AI was wrong. 

%The data-oriented process also help participants get more confidence in the result.  This gain in the sense of alignment between their expectation and what they see gradually increased confidence that AI is correct.

\subsubsection{Procedure Artifacts in Support of Validating the Data} 
\label{sec:results_procedure_support_data}
Within \dataworkflows~, we observed participants (10/22)  using procedure artifacts to support their data verification processes (13/52). Procedure artifacts enabled better comprehension of the data and even helped surface issues with the AI-generated analyses. 
% In many cases, noticing an issue in the AI's procedure  triggers participants to transitioned to a \dataworkflow~ from a \processworkflow~ to dig into the potential problem (see Table~\ref{tab:freq-of-workflows}) (P1, P2, P4, P5, P6, P12, P13, P14, P21, P22). For example, P2 transitioned to a \dataworkflow~ to better understand the data and see examples where the budget equals 1, as noted in the result of the AI's output. As illustrated in the second workflow in Figure \ref{fig:workflows}, P4 transitioned from \processworkflow~to a \dataworkflow~after noticing that the output is not sorted by flight code. Then P4 focused on verifying the result data table against AI's operation of taking the counts of flights to get confirmed that this is indeed the source of error. \ken{I'm not sure this fits since procedure comes before data}

Many participants used the NL explanation and code to help them understand the data and explain the relationships and values observed in the data tables (P1, P3, P13, P15, P16).  P1 in T2 is a typical example (Fig. \ref{fig:workflows} first row). P1 started out in a ~\processworkflow~but upon perceiving an issue in the original data table where more than 5 items had a rating of 5, transitioned into a \dataworkflow~. They scrutinized the original data table but became confused when the result data table displayed values less than 5. This contradicted their initial observation where more than five products had a 5 rating in the original data. To resolve this, they turned to the intermediate data and the AI's procedure, tracing the steps in the code that derived the result table. P3, meanwhile, first meticulously examined the original, intermediate, and result data to gain a comprehensive understanding of the AI-generated analysis. Upon noticing duplicates in the rank difference, in reference to the procedure artifacts, they remarked, \shortquote{I'll need to look into what it did.} 

Participants also noticed issues when using procedure artifacts to support their understanding of the data (P1, P9, P13, P15, P16, P17, P21). For instance, P17 wanted to explore why the intermediate data table contained all kinds of departure time. They checked the code to see where it did the filtering on the \textit{Departure Time} and realized the AI missed taking into account the time of the day when calculating the minimum of prices [T6]. In a few cases, participants became overconfident around the AI's correctness and subsequently formed an incorrect conclusion due to their reliance on verifying the data artifacts with the AI's procedure (P15, P17). In T5, P17 was initially skeptical of the result table due to insufficient information presented, yet gained confidence that the result \shortquote{looked more or less correct} after exploring and manipulating the data while cross referencing the AI's NL explanation and code. P15 manually reviewed the original data and formed expectations based on the AI's NL explanation and code. They confirmed that the AI is correct when the result data table matched their expected output [T1].

%Similarly, P1 used the code to pinpoint the error source that the output data was wrong because the code wasn't retrieving any data for \shortquote{Gourmet \& World Food} but only for \shortquote{Gourmet}. 

%Furthermore, checking the procedure artifacts to better understand the data artifacts in \dataworkflows~helped participants develop confidence.    % P1 used the code to pinpoint the error source that the output data was wrong because it wasn't retrieving any data for \shortquote{Gourmet \& World Food} but only for \shortquote{Gourmet}. 



%\subsection{\rqArtifacts} 
%\subsubsection{Process-Oriented Artifacts} 
%Participants' preferences towards code varied. Some participants, like P14 and P5, found the code interesting and important. P14 stated, \shortquote{I think the data table and the code was the most interesting.} However, others like P1 and P12 found the code difficult to read or not helpful. P1 stated, \shortquote{So I thought the code was helpful, but I also felt like it was kind of chunked up in a way that was not easy to read.} In one of the tasks \anna{cite task}, P19 mentioned, \shortquote{In this second example where if I could kind of deduce like what went right or wrong outside of code, then I'm not gonna bother looking at the code because the code is the code, whatever.}

%Some participants, like P12 and P21, preferred the NL summary and explanations over the code. Participant P15, for instance, used the comments as a reference point to confirm their understanding of the code. They stated, \shortquote{when I looked at the code and I would go back to the comments and say, OK, yes, my interpretation of what that code is doing aligns with the comment.}  P12 stated, \shortquote{For me it's more clear to have it communicated back to me in a very concrete and precise way that makes sense to me and maybe some people think in code like all the time and that's how they check code.} P21 echoed this sentiment, stating, \shortquote{I would probably default to the English or the high level summary translation and that would probably be fine. But you know, for some tasks I think it would be easier to look at it in code and things like that.}%Participants also use additional artifacts to veify the code. A few participants (P1, P11, and P15) use the code comments to interpret the steps and data operations. Some other participants make use of data tables and output to verify the code (P20, P3). For example, P20 went back and forth between the code and table to verify the process, stating, \shortquote{just like understanding what the code did and then each of the intermediate steps in seeing like ... it looks like it joined it.} Others use the code to check the logic of AI's procedure (P4 and P6). In particular, P6 expected to see some outputs at the end of thei inspection of logic, \shortquote{It kind of helped me see what logic it followed, but at the end of it, I'm like, OK, show me the numbers.} 

%\subsubsection{Data-Oriented Artifacts}
%\paragraph{Data tables} Participants' interaction with the data table artifact provided in the UI varied, with some finding it useful while others did not. However, a common theme was the trust participants placed in the data tables as a source of truth. For instance, P21, working with the Netflix dataset, decided to trust the data and the intermediate steps over the code, stating, \shortquote{I have decided not to go with the code and to trust what I see in the data and the intermediate steps.} 

%Participants' comfort with data tables also influenced their interaction with this artifact. P9 focused on the data tables, explaining, \shortquote{I guess that's probably because that's what I'm comfortable with.} Similarly, P16 found comfort in data tables, stating that they were essentially doing a lot of data comparisons to see if the results made sense based on their knowledge.

%The usefulness of data tables was generally acknowledged by participants. P6 found the data tables useful, while P17 and P18 found the intermediate data tables particularly helpful. P17 used the category to confirm if the filtering was correct, and P18, working with the Netflix dataset, stated, \shortquote{The merged dataset is the most interesting dataset for me.} However, not all participants found the intermediate data tables useful. P11 did not look at the intermediate tables at all, focusing instead on whether the AI reached the correct answer. They stated, \shortquote{So like it gave those intermediate tables and you saw didn't look at them at all because to me it was, you know, did it get to the right answer?} Similarly, P22 did not find the intermediate data table helpful in one of the tasks (movie content).

%\paragraph{Summary visualizations}
%Several participants expressed appreciation for the data table summary and visualizations provided in the AI's procedure (P5, P7, P13, P17, P20) (P5, . For instance, P5 emphasized the importance of code and visualization in their workflow, stating, \shortquote{I think the code and visualization are the most important things.} P7 made good use of the data summary to understand the data, expressing that, \longquote{And then definitely the summary stats to be able to do a quick view of the data and understand what it is instead of me having to manually check everything. So that really helped with the verification.} P20 also expressed a liking for the visualization provided. P13 appreciated the summary and visualization but still preferred familiar tools, stating, \longquote{Summary of visualization is good. Nice to have it. But might not necessarily need it all the time because I would do my own summary in Excel.}

%Some participants used the visualization to surface issues and validate steps.  P17 found the summary of the intermediate dataset helpful, using it to confirm if the filtering in the last step was correct. P5 also found the summaries of the intermediate datasets helpful for verification, stating, \shortquote{The fact that you provided summaries here with the intermediate datasets helps to validate it.}

% \subsubsection{Needs and Wants}
% \ken{TODO}
\subsection{Background Impact on Workflows and Artifacts Used}
\label{sec:results_bg}
In the post-task interviews, we explored participants' prior experiences with data analysis, coding, and existing analysis tools. We observed a range of experiences that influenced participants' approaches, workflows, and  interactions with different artifacts to verify AI-generated data analyses.

\subsubsection{Prior Experience With Data}
Participants sometimes attributed their focus around \dataworkflows~to their prior experience working with data (P6, P9, P11, P16, P17, P18, P22). For instance, P15, who had previous experience working with large datasets, expressed comfort with directly manipulating the datasets, stating, \shortquote{I'm used to working with hundreds of thousands of rows, so the size of the spreadsheet wouldn't have been a problem.} In both tasks P15 did, they only followed \dataworkflows~. These prior analysis experiences also led analysts to be vigilant about the data (P6, P9, P11, P22). P6, who self-identified as a \shortquote{data guy}, was inclined to dive directly into the data and scrutinize the tables and numbers. P11, an electrical engineer by training, also favored a data-oriented approach. 
 % His career in system design had honed his problem-solving skills, leading him to always start with clarifying the problem at hand and his existing knowledge around it. 
 They compared the study tasks to their past experiences designing systems, explaining how they always \shortquote{went straight to the data} and asked \shortquote{hey, can I trust that it's quality data?}
 % P22, drawing from their prior experience, emphasized the importance of correctly cleaning the data, stating \shortquote{I'm gonna filter out the data with wrong values and that should be a huge red flag in any data analysis.} 
 % P17, an experienced data scientist, also extensively utilized the \dataworkflow~ in her process, stating \shortquote{If I've had this answer from either my intern or my AI tool, I would have felt the urge to go and work on the data myself.} 
 P9, with a background in finance and accounting, was accustomed to handling datasets that were \shortquote{routinely between 100 and 500,000 rows.} In the study, P9 focused on validating the data, underscoring the importance of ensuring data integrity and rational calculations. Similarly, P22  cited their  prior work experiences as informing their analysis verification approach: \shortquote{we were maniacal about not drawing the wrong conclusion.} During their verification process, they demonstrated a methodical approach to problem-solving, routinely considering \shortquote{lots of caveats and checks.}  

Moreover, we noticed participants' prior experiences forming conclusions and insights from data shaped their behavior in the study tasks. Participants started the verification processes by proactively devising their own analysis plan. A few participants participants (P1, P6, P9, P19, P22) mentioning being accustomed to formulating error hypotheses, setting expectations, and actively identifying problems in the data. For example, P19 commented how in their own data analysis workflow they were always on the lookout for \shortquote{weird stuffs} like data classes, data types, and anomalies. This was reflected in their systematic verification process when faced with our study tasks.


\subsubsection{Prior Experience With Code}
\label{sec:results_bg_code}
While participants' experiences working with data sometimes led them to being more data-oriented, a couple participants' coding comfort made them inclined to follow procedure-oriented workflows specifically through the code (P5, P8). For instance, P8, a software engineer, naturally tried to verify the correctness of the code: \shortquote{as a developer, just let me look at the code.} Similarly, P5, compared the tasks to doing a \shortquote{code review.}

Interestingly, participants who were not familiar or comfortable with Python but had a familiarly of data operations and/or data-oriented programming languages (e.g., SQL and Visual Basics for Applications) managed to leverage their knowledge to understand the AI's procedure on the data (P10, P15, P19, P20, P21). For example, P4 looked for key words in the code to understand the the AI's operations. For P10 in T9, despite having no prior experience with Python, they were able to devise the analysis steps in SQL and cross-check them against the AI's explanation and code comments: \longquote{If I were to do this in SQL Server with the table that you gave me, I would have created ... select unique \Asterisk ID where director and popped the table out ... So basically, I'm translating Python into the technologies I know to see if the AI is doing what I need them to do.} 

However, while able to parse key words or main points from the code, a lack of understanding of the code hindered some participants' confidence in their verification process (P2, P12, P14, P18, P20, P21). For example, P20 found T5 \shortquote{difficult because (they didn't) fully understand the code.}
For P18, an incomplete comprehension in T9 led them to focus more on the original data as opposed to the intermediate data since they were unsure how the intermediate data was generated: \shortquote{in the intermediate steps, I am not confident if the slicing and the dicing is being done the way it should be.} To bridge this gap, a couple participants mentioned liking code documentation or being able to easily translate the code to a more familiar languages (P11, P21). 


\subsubsection{Prior Experience With Existing Analysis Tools}
\label{sec:results_bg_tools}

% Integrate with familiar tools like Excel
Our study aimed to include participants with a diverse usage of existing analysis tools~(Table~\ref{tab:participants}).  While there were ways to verify the AI-generated output using our design probe~(Fig.~\ref{fig:interface}), some participants expressed a preference for functionality they were familiar with from existing tools that were unsupported by our interface (P12, P13, P15, P18, P21). For example, P12 mentioned wanting to use conditional sorting on the columns, and P17 wanted support for  comparison operators in data filtering. Several participants also expressed a desire to have pivot tables (P11, P17, P18, P21), making it easier to understand the data. Moreover, while many participants expressed appreciation for the visual summaries of the data tables (P5, P7, P13, P17, P20), P21 expressed low trust in the artifact because they were unsure how the artifacts were created in the first place. They felt more comfortable with using more familiar tools: \longquote{The (visualization) summary tab was kind of useless to me... I didn't really trust it and and it was unclear to me how the the data was being summarized.}
% In addition, with the exception of P22 (whose work involves building AI-based products), participants in our study had not extensively used AI-based analysis assistants (unsurprising given the infancy of such assistants). Those who had experiences with AI assistants used them for writing (P13, P20), answering questions (P8), programming (P11), and casual experimenting (P7, P8, P10). Informed by prior experiences where general AI-based assistants (e.g., ChatGPT~\cite{ChatGPT}) failed,  some participants express distrust towards an AI performing data analysis goals  (P10, P11, P12, P15, P20, P21). During the study, a few participants were surprised and impressed by AI's reasoning ability around data analysis, such as interpreting meaning of under-specified columns, articulating concerns around outputs and offering mitigation strategies (P6, P19, P22). 


% In addition, We found that none of our participants has used LLMs extensively for any data analytical tasks. One exception is P22, whose have been involved in building products with LLMs. Participants have only used LLMs for writing purposes (P13, P20), Q\&A (P8), programming (P11), and casual experimenting (P7, P8, P10).

% Besides analytical and programming experience, interestingly, non-technical skills were also crucially helpful in detecting AI's source of error. As a program manager with a technical background, P12 said a big part of her work is communicating with people. She had strong intuition about what AI might go wrong in its analysis process just based on AI's description of its understanding of the data or its process. She connected this to her experience learning where communication can break down, and she thinks that AI might do the analytical task wrong because language inherently carries a huge amount of ambiguity.

% While many participants preferred to manually verify the data before drawing conclusions about the AI's correctness (P3, P7, P9, P13, P18, and P19), their reliance on the AI varied in terms of methods and degrees. Some participants expressed a desire to verify the results by executing queries in their own environments. For instance, P1, a data scientist, stated that they does not even trust his own work without verification and double-checking. Consequently, P1 preferred to maintain agency over the results by executing the code generated by the AI himself. 

%Commenting on the AI showing its process, P22 also stressed the importance of \shortquote{show your work} as a part of the training as a data scientist. 
%Participants who have strong data science background tend to be more familiar with the analysis procedure and data operations. We observed that these participants would first articulate the steps and then adopte data-oriented workflow to manipulate the data on their own following their own procedure and then verify with the AI's output. 

% Reliance on AI: On the other hand, participants like P6 and P8, who have decent understanding of code, wanted the AI to guide them partially through the process but preferred to finalize the process themselves.


==> 7-results.tex <==


\workflowsFig
\casesFig

\section{Results}
\label{sec:results}

% \ken{Branching \cite{Jiang2023GraphologueEL, Suh2023SensecapeEM}}

Participants engaged in a variety of different steps to identify potential issues and ultimately confirm or reject the AI's analysis. These were guided by two high-level \behaviors participants had within a verification workflow:~\textit{procedure-oriented \behaviors} and \textit{data-oriented \behaviors}~(Fig.~\ref{fig:workflows}).

Within a verification workflow, participants with \processworkflows~were primarily focused on validating the AI's procedure, possibly drawing upon data artifacts to aid their understanding. In contrast, participants exhibiting \dataworkflows~gave precedence to scrutinizing the data involved in the analysis, relegating the AI's procedure to a supplementary role. The distinction between these \behaviors lies in the participants' intention. Participants following \processworkflows were concerned with \textit{what does the AI do?} Meanwhile participants following \dataworkflows focused on \textit{does the data make sense?} This was clear from observing their interaction patterns and verbal comments. For example, while some participants engaged extensively with intermediate datasets, their main goal in those moments was to confirm the correctness of the AI's procedure; this behavior was labeled as a \processworkflow with the use of data artifacts as secondary support (i.e., \process~).
% Given these \behaviors, participants typically started with \processworkflows and diverged when faced with an issue (\textbf{RQ1}) (see Fig.~\ref{fig:cases} for examples). Within these \behaviors, participants leveraged both data and procedure artifacts, not only as central elements in their primary intent but also as supporting artifacts to both reinforce their comprehension and validation (Fig.~\ref{fig:artifacts}) (\textbf{RQ2}). From our post-task interviews, we observed how participants' backgrounds influenced them towards ~\dataworkflows~or \processworkflows~and how a familiarity with data operations and basic programming helped them understand the AI's procedure (\textbf{RQ3}).
In this section, we provide a detailed account of findings pertinent to our research questions.

\subsection{\rqWorkflows}
\label{sec:results_workflow}

Overall, we observed most participants (18/22) followed all or parts of the AI's procedure at some point during their verification workflows (44/52). In workflows in which participants did not follow the AI's procedure, they only used the analysis goal, intern's prompt, and data (original and intermediate) artifacts. Likewise, most participants (18/22) had \dataworkflows in their verification workflows (25/52). Participants generally exhibited different behaviors at different moments in their workflows to focus on different parts of the AI-generated response.

\subsubsection{Analysts initially gravitate toward \processworkflows}
Participants usually had \processworkflows~initially during their verification workflows (41/52). These \behaviors were relatively time-consuming and similar to when programmers thoroughly examine the code's logic when they validate suggestions from an AI programming assistant. However, in contrast to the programming assistant setting, \processworkflows were rarely as brief as the quick verification methods (e.g., visual inspection and pattern matching) programmers most commonly employ~\cite{Barke2022GroundedCH, Liang2023ALS}. 

\tableWorkflows

\subsubsection{Analysts shift toward \dataworkflows~ once they noticed an issue}
Upon identifying a concern, participants' strategies diversified, delving deeper to explore and validate the perceived issue~(Table~\ref{tab:freq-of-workflows}). Of the 31 times in which participants noticed an issue but had not yet confirmed an error, 17 times (15/22 participants) they continued their verification workflow with \dataworkflows. In particular, 13 of 17 of these occurrence were when participants switched from \processworkflows to \dataworkflows after noticing an issue.

Some participants (P2, P15, P16, P20, P22) identified the source of the issue through eyeballing different data tables, while others had ~\dataworkflows~to check more closely the potential source of an issue (P4, P5). In T2, P5 correctly noticed that there was no consideration for \textit{Nivea Men}. To explore this further, they focused on the original data table, filtering for rows in which the brand was \textit{Nivea} and applying additional filters to spot check specific products. Similarly, to affirm their suspicions of an error, P4 investigated the final result table after noticing the AI may not have grouped rows by \textit{flight code} (Fig.~\ref{fig:cases} second row) [T5]. 


\subsubsection{Analysts adopt \processworkflows~to get a high-level understanding of the analysis steps}
\label{sec:results_rq1_procedure_high}

 Many participants looked over the AI's procedure to get a high-level understanding of the analysis steps (P1, P2, P4, P8, P11, P17, P18, P20). For instance, in T9, P18 wanted to understand how the AI arrived at a particular actor-director pair in the result: \shortquote{I'm trying to read the code and I'm trying to understand ... like how is it generating that pair and if there is any error in that process.} Sometimes, participants gained confidence in the AI's correctness
% \steve{I noticed this in many places, you should probably nearly always use an article in front of AI - the AI's correctness - in this case, but many times you don't} 
from this high-level understanding  (P1, P2, P11, P20). For example, P1 confirmed their understanding after reading the AI's  procedure one last time:~\shortquote{seems reasonable to me.} P11 was reassured by the AI's overall procedure matching their own:~\shortquote{the steps it described is exactly what I would have done but in SQL.} In other cases, participants' focus on the procedure helped them notice and subsequently confirm a particular step the AI did wrong (P4, P8). For example, P4 and P8 both noticed from the NL explanation that the AI's order of analysis steps were incorrect [T5]. In T6, similar to P11, P4  broke down the general steps on their own and realized the AI missed calculating the average after inspecting the AI's procedure. 

\subsubsection{Analysts adopt \processworkflows~to confirm details in the data operations}
\label{sec:results_rq1_procedure_low}
Participants also focused on lower-level details involved in the AI's data operations  (P2, P7, P8, P9, P10, P11, P13, P15, P17, P22). Participants checked functions used in the code, logic around the data operations, and specific result values. P13 was especially vigilant making sure that \shortquote{the spelling was correct} in the data columns mentioned in the code, and that \shortquote{syntactically ... (they) appear to be correct.} P19 was also following the AI's data operations to see how it handled unusual values the AI had identified earlier in its procedure. Focusing on low-level details was one way participants gained confidence in the AI or noticed issues (P7, P8, P10, P11). For instance, in T9, P10 focused on the AI's data operations in the code which helped them conclude the AI had indeed found the highest count. P11, while not the most comfortable with Python, used code comments to translate the AI's procedure into familiar data operations, noticing the AI's procedure was inconsistent with the analysis goal description [T8].

However, participants sometimes formed incorrect conclusionsa due to their reliance on the AI's procedure (P15, P17). In T5, P17 was initially skeptical of the result table due to insufficient information presented, but gained confidence that the result \shortquote{looked more or less correct} after cross referencing the AI's NL explanation and code with the data. P15 manually reviewed the original data and used the AI's NL explanation and code to form an incorrect expectation of the output. They confirmed that the AI was correct when the result data table matched their expectation [T1].


\subsubsection{Analysts adopt \dataworkflows~to better understand the structure of and relationships in the data}
\label{sec:results_rq1_data}
Participants in \dataworkflows~focused on the data in a variety of ways. Some participants (P3, P7, P15, P19) were keen on understanding the data (original and intermediate) and the specific columns that were pertinent to the analysis goal. For instance, P7 adopted \dataworkflows~ using only data tables at the beginning of their process, exploring the column of interest in the analysis goal and subsequently identifying a data quality issue in the frequency column [T10]. Meanwhile, for P9, a prototypical data-oriented participant, their \dataworkflows~involved comparing all data tables [T9]. Specifically, they delved into the directors and actors intermediate data tables to gather an expectation of what they would expect in the subsequent merged data table (Fig.~\ref{fig:cases} third row). After, they checked if specific actors in the result data existed in the merged data. In the process, they spent significant time forming an expectation of the result data, transitioning back and forth between all data tables.


\subsection{\rqArtifacts}
\label{sec:results_artifacts}
\artifactsFig

Across all participants, both data and procedure artifacts were used consistently in their verification workflow (Fig.~\ref{fig:artifacts}). Data artifacts were frequently employed to support \processworkflows~(17/22 participants and in 41/52 workflows), while procedure artifacts were utilized during \dataworkflows (10/22 participants and in 13/52 workflows).  Within the data, participants engaged with the intermediate data roughly equally as often as the original data and result data. Similarly, for procedure artifacts, participants leveraged code and code comments as often as the natural language explanation. However, these preferences for artifacts were not consistent between participants (see Sec.~\ref{sec:results_bg}).

\subsubsection{Analysts use data artifacts for sensemaking}
\label{sec:results_rq2_data}
Unsurprisingly, most participants leveraged data artifacts to understand and interpret the data, a standard practice in data analysis practices~\cite{Alspaugh2019FutzingAM, Batch2018TheIV, Grolemund2014ACI}. For instance, P7 used the data summary visualizations to understand the data, and expressed liking \shortquote{the summary stats to be able to do a quick view of the data and understand what it is instead of having to manually check everything.} P3, meanwhile,  meticulously examined the original, intermediate, and result data to have a comprehensive understanding of the analysis. Consequently, several participants expressed appreciation for the data table summary and visualizations provided in the AI's procedure (P5, P7, P13, P17, P20).  

Through closely examining the data tables, participants were able to identify issues with the AI-generated analyses (P1, P3, P7, P9, P13, P15, P16). For instance, from the data tables, P1 noticed that there was also the \textit{Nivea Men} brand in the dataset which the AI missed (Fig.~\ref{fig:cases} first row), ultimately leading them to confirm that the AI-generated analysis contained an error. Likewise, for P9, their exploration of the data tables led them to perceive a discrepancy with the number of rows in merged data table and the count from a quick mental calculation. These observations align with established guidelines in data analysis practices and implementations of data analysis tools, and underscore the importance of data visualizations alongside the analysis procedure~\cite{Alspaugh2019FutzingAM, Kery2019TowardsEF, Choi2023TowardsTR, Batch2018TheIV, Kery2018InteractionsFU, Wu2020B2BC, Moritz2017TrustBV} . 


\subsubsection{Analysts frequently use data artifacts for both quick checks and detailed calculations to support \processworkflows}
\label{sec:results_rq2_data_support_procedure}

Some participants glanced at the data artifacts to quickly check things they noticed in the AI's procedure (P6, P8, P22). For instance, P22 noticed that the AI's calculation for the average price of gourmet food was not a number, prompting them to check the original data table and discover the AI used the wrong column name [T2]. Similarly, participants used data artifacts to conduct data sanity checks to verify the procedure (P1, P3, P4, P5, P19, P20, P21, P22). For instance, P19 wanted to see if percentages in a column added up to 100: \shortquote{If the percentages tied to 100\%, I would feel confident just at a glance that you know everything and action was allocated to one of those languages} [T8]. P20, meanwhile, went back and forth between the code and table to verify the procedure, stating, \shortquote{just like understanding what the code did and then each of the intermediate steps in seeing like ... it looks like it joined it} [T6].
Alternatively, participants also tried to replicate the AI's data operations using the supported functionalities in the data tables to compare with the result in the AI's procedure and verify what the AI did (P2, P9, P12, P14, P22). For example, P22 filtered on the \textit{frequency} column following the AI's steps to see how many rows were filtered out [T10]. 

These approaches align with common AI-assisted programming verification methods~\cite{Liang2023ALS, Barke2022GroundedCH}, resembling visual inspection and pattern matching for quick data checks, and code execution for replicating the AI's data operations. However, distinct from AI-assisted programming, data (in addition the procedure) serves as a central artifact for verification.


\subsubsection{Analysts use procedure artifacts to find discrepancies in the procedure}
\label{sec:results_rq2_procedure}

Some participants were keen on verifying the consistency between the high-level analysis steps in the NL explanation and the specific data operations in the code (P5, P11, P17, P22). Meanwhile, other participants compared the NL explanation with their own common knowledge. For example, P10 felt that \shortquote{2800 flights felt like a lot} for a day [T5], leading them to investigate the AI's procedure. Similarly, from inspecting the AI's explanation of the result, P6 noticed \shortquote{Jurassic World is not a Bollywood movie} [T4]. These discrepancies prompted them to question the AI's data operations and understanding of the dataset. Moreover, participants used procedure artifacts to verify the AI's interpretation of the prompt and original dataset (P4, P12). As a result, in T7, both P4 and P12 noticed issues with the AI's understanding of the data, stating an incorrect interpretation of a column. 

\subsubsection{Analysts use procedure artifacts for tracing data provenance to support \dataworkflows}
\label{sec:results_rq2_procedure_support_data}
Many participants (P1, P3, P13, P15, P16) used the NL explanation and code to trace the provenance of data. P1 in T2 is a typical example (Fig. \ref{fig:cases} first row). P1 started out with~\processworkflows~but upon perceiving an issue in the original data table where more than 5 items had a rating of 5, transitioned into \dataworkflows. They scrutinized the original data table but became confused when the result data table displayed values less than 5. This contradicted their initial observation where more than five products had a 5 rating in the original data. To resolve this, they turned to the intermediate data and the AI's procedure, tracing the steps in the code that derived the result table. 

Participants also noticed issues when using procedure artifacts to support their understanding of the provenance of the data (P1, P9, P13, P15, P16, P17, P21). For instance, P17 wanted to explore why the intermediate data table contained all kinds of departure time. They checked the code to see where it did the filtering on the \textit{Departure Time} and realized the AI missed taking into account the time of the day when calculating the minimum of prices [T6]. These behaviors reiterate the importance of tracking data provenance in analysis tools and highlight opportunities to adopt and adapt methods in existing implementations~\cite{Kery2017VarioliteSE, Rule2018AidingCR, Kery2018TheSI, Wang2022DiffIT, Pu2021DatamationsAE, Wu2020B2BC, Park2021StoryFacetsAD}.


\subsection{\rqBackground}
\label{sec:results_bg}
In the post-task interviews, we explored participants' prior experiences with data analysis, coding, and existing analysis tools. We noted a range of experiences that might be associated with participants' behaviors and interactions with artifacts.

\subsubsection{Prior Experience With Data}
\label{sec:results_bg_data}

Some participants with \dataworkflows~ mentioned their prior experience working with data (P6, P9, P11, P16, P17, P18, P22). For instance, P15, who had previous experience working with large datasets, expressed comfort with directly manipulating the datasets, stating, \shortquote{I'm used to working with hundreds of thousands of rows, so the size of the spreadsheet wouldn't have been a problem.} In both tasks P15 did, they only followed \dataworkflows. 

These prior analysis experiences also led participants to be vigilant about the data (P6, P9, P11, P22). P6, who self-identified as a \shortquote{data guy}, was inclined to dive directly into the data and scrutinize the tables and numbers. P11, an electrical engineer by training, also favored a data-oriented approach. 
 % His career in system design had honed his problem-solving skills, leading him to always start with clarifying the problem at hand and his existing knowledge around it. 
 They compared the study tasks to their past experiences designing systems, explaining how they always \shortquote{went straight to the data} and asked \shortquote{hey, can I trust that it's quality data?}
 % P22, drawing from their prior experience, emphasized the importance of correctly cleaning the data, stating \shortquote{I'm gonna filter out the data with wrong values and that should be a huge red flag in any data analysis.} 
 % P17, an experienced data scientist, also extensively utilized the \dataworkflow~ in her process, stating \shortquote{If I've had this answer from either my intern or my AI tool, I would have felt the urge to go and work on the data myself.} 
 P9, with a background in finance and accounting, was accustomed to handling datasets that were \shortquote{routinely between 100 and 500,000 rows.} In the study, P9 focused on validating the data, underscoring the importance of ensuring data integrity and rational calculations. Similarly, P22  cited their  prior work experiences as informing their analysis verification approach: \shortquote{we were maniacal about not drawing the wrong conclusion.} During their verification workflows, they demonstrated a methodical approach to problem-solving, routinely considering \shortquote{lots of caveats and checks.}  
%Participants' comfort with data tables also influenced their interaction with this artifact. P9 focused on the data tables, explaining, \shortquote{I guess that's probably because that's what I'm comfortable with.} Similarly, P16 found comfort in data tables, stating that they were essentially doing a lot of data comparisons to see if the results made sense based on their knowledge.

Moreover, we noticed participants' prior experiences forming conclusions and insights from data shaped their behavior in the study tasks. Participants  (P1, P6, P9, P19, P22) who started their verification workflow by proactively devising a plan mentioned being accustomed to formulating error hypotheses, setting expectations, and actively identifying problems in the data. For example, P19 commented how in their own data analysis workflow they were always on the lookout for \shortquote{weird stuffs} like data classes, data types, and anomalies. This was reflected in their systematic approach when faced with our study tasks.


\subsubsection{Prior Experience With Code}
\label{sec:results_bg_code}
While participants' experiences working with data sometimes led them to being more data-oriented, a couple participants' coding comfort made them inclined towards \processworkflows and examining the code (P5, P8). For instance, P8, a software engineer, naturally tried to verify the correctness of the code: \shortquote{as a developer, just let me look at the code.} Similarly, P5, compared the tasks to doing a \shortquote{code review.}
Interestingly, participants who were not familiar or comfortable with Python but had a familiarity of data operations and/or data-oriented programming languages (e.g., SQL and Visual Basics for Applications) managed to leverage their knowledge to understand the AI's procedure on the data (P10, P15, P19, P20, P21). For example, P4 looked for key words in the code to understand the the AI's operations. For P10 in T9, despite having no prior experience with Python, they were able to devise the analysis steps in SQL and cross-check them against the AI's explanation and code comments: \longquote{If I were to do this in SQL Server with the table that you gave me, I would have created ... select unique ID where director and popped the table out ... So basically, I'm translating Python into the technologies I know to see if the AI is doing what I need them to do.} 

However, while able to parse key words or main points from the code, a lack of understanding of the code hindered some participants' confidence (P2, P12, P14, P18, P20, P21). For example, P20 found T5 \shortquote{difficult because (they didn't) fully understand the code.}
For P18, an incomplete comprehension in T9 led them to focus more on the original data as opposed to the intermediate data since they were unsure how the intermediate data was generated: \shortquote{in the intermediate steps, I am not confident if the slicing and the dicing is being done the way it should be.} To bridge this gap, a couple participants mentioned liking code documentation or being able to easily translate the code to a more familiar languages (P11, P21). For P12 and P21 in particular, a lack of code comprehension led them to prefer the NL explanations over the code. P12 found the explanations to be \shortquote{a very concrete and precise way that makes sense.}


\subsubsection{Prior Experience With Existing Analysis Tools}
\label{sec:results_bg_tools}

% Integrate with familiar tools like Excel
Our study aimed to include participants with a diverse usage of existing analysis tools~(Table~\ref{tab:participants}).  While there were ways to verify the AI-generated output using our design probe~(Fig.~\ref{fig:interface}), some participants expressed a preference for functionality they were familiar with from existing tools that were unsupported by our interface (P12, P13, P15, P18, P21). For example, P12 mentioned wanting to use conditional sorting on the columns, and P17 wanted support for  comparison operators in data filtering. Several participants also expressed a desire to have pivot tables (P11, P17, P18, P21), making it easier to understand the data. Moreover, while many participants expressed appreciation for the visual summaries of the data tables (P5, P7, P13, P17, P20), some participants (P4, P18, P21) expressed low trust in the data artifacts because they were unsure how the artifacts were created in the first place. P21 in particular stated: \longquote{The (visualization) summary tab was kind of useless to me... I didn't really trust it and and it was unclear to me how the the data was being summarized.}


==> 8-discussion-future-work-submission.tex <==
\section{Discussion}
\label{sec:discussion}
In this work, we examined how data analysts understand and verify AI-generated analyses. We developed a design probe, prepared realistic analysis queries and AI-generated analyses, and conducted a user study observing analysts' verification processes and common workflow patterns. In this section, we synthesize the results from our user study and share implications for data analysts using AI-based analysis tools (Sec.~\ref{sec:discussion_impl_analyst}) and system designers building these tools (Sec.~\ref{sec:discussion_impl_designers}).


\subsection{Implications for Data Analysts}
\label{sec:discussion_impl_analyst}
\subsubsection{The Role of Data Literacy in Analysis Verification}
\label{sec:discussion_impl_analyst_data_lit}
Our findings suggest that while a lack of familiarity with one particular programming language (in this case Python) is not a barrier for verifying AI-generated analysis, prior experience with data operations in other languages (e.g., SQL or Visual Basics for Applications) can aid in understanding the AI's procedure (Sec.~\ref{sec:results_bg_code}). Likewise, knowledge and experience in data analysis are often indispensable for grasping AI-generated analyses. This mirrors the requirement for computational thinking skills when working with AI-based code assistants~\cite{Sarkar2022WhatII}. Here, we highlight two recommendations for analysts to be more effective in verifying AI-generated analyses.

% We found that even for experienced data scientists and analysts, they actively engage with both the procedure and datasets to identify the potential issues in AI's results (Sec.~\ref{sec:results}).

\yhdr{Know Common Data Operations} In the verification process, we observed participants closely examined the AI's data operations and sometimes performed these operations on the datasets directly to compare with AI's result (Sec.~\ref{sec:results_data_support_procedure} and 
 Sec.~\ref{sec:results_dworkflow}). This involved understanding common operations such as filtering, sorting, and merging the data. Similarly, understanding aggregation operations, such as sum, average, count, were also essential to verify how the AI grouped data and performed calculations on those groups. Therefore, analysts should understand the data operations essential in both data-oriented and process-oriented workflows.

% In addition, analysts should also be familiar with some common ways to handle data quality issues. For example, in T10, the analyst should know ways of missing values to tell that the AI forgot to check the other columns which might contain values to fill in.

\yhdr{Develop Strategies for Quick Data Validations} Our observations revealed analysts often employed quick sanity checks on the data (e.g., eyeballing values, manual summation of rows, using visualizations to check the value distributions, spot checking result values against original data table, and comparing things against common knowledge) as a strategy to assess the AI-generated outputs (Sec.~\ref{sec:results_data_support_procedure} and Sec.~\ref{sec:results_focal_in_data}). These were effective for analysts to either build confidence in the results or identify unexpected patterns. The sanity checks often involved forming expectations around the result and then comparing them with the AI-generated output. Any discrepancies signaled potential issues that demanded further inspection.
% For example, in T2, analysts can quickly check if the result table contains both \textit{nivea} and \textit{nivea men} by filter the original data table with these values and sum the rows of the filtered datasets and compare with the result table to notice that AI didn't account for ``Nivea Men" in its result. 
Given the effectiveness, analysts should use quick sanity checks in their verification process. However, as there may be data issues hidden by seemingly reasonable patterns~\cite{correll2018looks}, analysts should employ a variety of different sanity checks.




\subsubsection{The Role of AI Assistants in Data Analysis}
\label{sec:discussion_impl_analyst_ai}
% LLM-powered data analysis is very new, people need to better understand how to make use of it
% we want people to understand the strengths and shortcomings at least in the 10 tasks and 50+ verification processes

% Participants generally entered our study tasks, skepti specifics of the AI's procedures and attempted to verify them (e.g., by ensuring the code performed as indicated in the comments), many ultimately expressed trust in the AI's overall analyses. They attributed the errors to the underspecification of the dataset or analysis goals (P1, P4, P6, P9, P10, P11, P12, P15, P19, P20, P22). A few of them noted that the AI did what it was asked for by the intern (P11, P19, P22). This suggests that analysts can leverage the AI’s strengths by shifting more of their attention from checking the low-level specifics to higher-level aspects such as the order of steps, whether the AI interpreted the task correctly, and if the AI has accurate knowledge about the data. This shift could potentially increase efficiency and accuracy in the verification process. To illustrate this idea in an example from the study, we observed that P12 was able to detect AI's error directly from its description of data and procedure. Rather than focusing on the technical details, they focused on detecting where the communication might fail between the AI and the intern who wrote the prompt, as she stated \shortquote{language inherently carries a huge amount of ambiguity.} The interaction paradigm between the analyst and the AI should be one where the human retains agency in verifying AI's reasoning and understanding and delegate AI assistants to perform the low-level tasks. \ken{Todo: cite paper related to division of agency between human and AI in data analysis}. The AI should be viewed as an intern that is proficient in low-level operations and coding but may overlook certain task goals and purposes due to ambiguity in communication or lack of context. 

Participants' varied experiences working with data and analysis tools (Sec.~\ref{sec:results_bg}) combined with their observations of AI analysis assistants' strengths and shortcomings in our study, led to a wide range of comments about their preferred use of general AI-based analysis assistants. Here, we discuss how AI assistants could be used in data analysis.

Some participants commented how AI-assistance would be helpful for getting them a partial answer that might guide them in their analysis process (P1, P6, P7, P14, P20, P21). For instance, P6 mentioned how the AI can help them consider alternative steps: \shortquote{It'll help me say `oh maybe didn't think of this way of solving this and I can now go down that path.'} AI assistants can help inspire ideas for analysis steps similar to when programmers follow an exploration mode  in AI-assisted programming~\cite{Barke2022GroundedCH}. Presenting alternative approaches is especially critical in analysis assistance as analysts can often be limited in their consideration of analysis approaches~\cite{Liu2019PathsEP, Liu2020UnderstandingTR}, thereby affecting the robustness of their subsequent analysis conclusions~\cite{Silberzahn2018ManyAO, Breznau2022ObservingMR, Schweinsberg2021SameDD}. Thus, AI analysis assistance can improve analysis quality by broadening the analysis decision space analysts consider ~\cite{Liu2019PathsEP, Gu2022UnderstandingAS}. 
% \tim{you should cite your own multiverse paper :D}

Similarly, participants noted that assistants can expedite their analysis process (P1, P13, P20), corroborating the findings from prior research on AI-code assistants ~\cite{Vaithilingam2022ExpectationVE, Ziegler2022ProductivityAO, Dibia2022AligningOM, GitHubCopilotResearch}. However, to ensure the robustness of the analysis conclusions, it is crucial to balance the acceleration of analysis with measures that surface potential errors, underlying data assumptions, and alternative approaches.

Finally, some participants expressed a preference to reserve AI assistance for peripheral tasks such as error-checking or report generation, rather than the central analysis process. Utilizing AI assistance in crafting reports~\cite{Zheng2022TellingSF, Wang2023Slide4NCP} and similar subsidiary activities offers a low stakes environment for analysts to evaluate the quality of AI-generated outputs within data analysis workflows. This approach can also facilitate a deeper understanding of the assistant's capabilities and limitations.

\subsubsection{Understand the Bounds of the AI and the Tool}

Participants (P4, P18, P21) sometimes expressed doubt on the intermediate data and even the summary visualizations as it was unclear what artifacts had the potential to be a result of AI ``hallucinations"~\cite{Ji2022SurveyOH} and which were consistent with regards to the data and procedure (Sec.~\ref{sec:results_procedure_support_data}). As the boundary blurs between AI-generated artifacts and tool-generated artifacts, analysts should clearly distinguish what is and what is not produced by AI.

Tool artifacts compiled from code is deterministic (i.e., the same summary visualization will be produced given the same code and input data)~\cite{Sarkar2022WhatII}. The AI-generated outputs and their associated errors are stochastic in nature, varying each time the AI is prompted to conduct the analyis. Knowing the provenance of artifacts used to support verification---what is tool-generated (e.g., the visual summary of data) and AI-generated (e.g., the intermediate data feeding into the visualization)---is important to assess the reliability of the information associated with these artifacts. Additionally, understanding the strengths and limitations of the AI~\cite{Ragavan2022GridBookNL, Sun2022InvestigatingEO} is crucial to knowing what types of AI-assistant mistakes to look for.

% More broadly, as analysts are likely to edit upon AI-generated output and share work that are collaborated with AI to others, it may be important for everyone involved to know what parts came from where. While prior work found data scientists did not view documentation of interactions with AI-based code assistants as important within computational notebooks~\cite{Mcnutt2023OnTD}, it is unclear whether this also applies to data artifacts and higher-level AI-generated analyses. For instance, given that several participants were maniacal about checking the data \ref{sec:results_focal_in_data}, would knowing the intern's history of back-and-forth prompts, checks on the data table and distinctly separating this from the AI-generated analysis help reviewers or audiences of such AI-assisted analyses? We leave this as important considerations for future work.

% Despite our participants being generally cautious and skeptical due to their prior data analysis experience and the study's setup, some still became overconfident in the AI's process and overlooked errors \ref{sec:results_procedure_support_data}. This overconfidence could stem from their unfamiliarity with the kinds of mistakes AI can make amidst the array of information AI generated in its analysis output.


% Knowing the provenance of artifacts and components between what the AI writes, what the tool includes, and humans. 

% Overall, AI-assistance can impact data analysis in a variety of ways


% In the study tasks, we identified several specific advantages of AI-assisted data analysis. First, AI-generated analyses proposed data operations that participants acknowledged they might not have thought of. The is similar to the exploration mode in found in AI-assisted programming~\cite{Barke2022GroundedCH}.The occasional times the AI assistant mentioned its interpretation of the data and reflection of potential missteps helped analysts deduce the source of errors from unexpected outputs. For example, in T3, the AI was able to notice the \textit{nan} values in the result and propose that this might be due to the wrong query used for filtering the data. Additionally, AI assistants could enumerate their assumptions about the data being used, thereby helping analysts identify misunderstandings and data quality issues, such as poorly labeled columns [T7].

%Interestingly, among the tasks that we used for the study, AI rarely made mistakes in the alignment between steps and operations versus the actual code and execution. If we view the procedure and outputs generated by the AI can be viewed as a series of translation from high-level stages to low-level details between task, steps, operations, code, original datasets, and output datasets, the analyst should actively examine the accuracy of translation between each two stages.




\subsection{Implications for System Designers}
Informed by our study findings of verification workflows and noted challenges, we highlight three design implications for designers of AI-based analysis assistants. 

\label{sec:discussion_impl_designers}
\subsubsection{Connecting data-oriented and procedure-oriented artifacts}
Our study on analysts' verification processes revealed that analysts often followed both data-oriented and procedure-oriented workflows. Data artifacts were often leveraged to support analysts' understanding of the procedure~(Sec.~\ref{sec:results_data_support_procedure}) and procedure artifacts were used to support analysts' verification of the data~(Sec.~\ref{sec:results_procedure_support_data}). The use of data-oriented and procedure-oriented artifacts were often intimately tied to each other, requiring analyst to switch between the two (e.g., intermediate data table and the code snippet that generated this data). Therefore, to support analysts' behavioral patterns, tools should support both data-oriented and procedure-oriented workflows and enable seamless transition between data  and procedure artifacts. Pointing to a specific step in the procedure should present the associated data artifact and vice versa.

As participants in our study often sought familiar operations in their verification process~(Sec.~\ref{sec:results_bg_tools}), these considerations can be integrated into existing tools considering their current capabilities and shortcomings. For example, tools like Code Interpreter~\cite{openai_codeinterpreter} and AI Coding in Google Colab~\cite{PerryMallick2023} are primarily centered around procedure-oriented verification workflows. Enhancing them with features that allow for easy reference and manipulation of data artifacts, like intermediate data tables or simple data visualizations, could be beneficial. Nevertheless, integrating these features may be challenging for all data workflows. It may not be easy to manipulate or visualize large datasets (i.e., with millions of rows)~\cite{Chattopadhyay2020WhatsWW}.


On the other hand, platforms that are more data-centric, such as spreadsheet environments, should provide interface elements that articulate the underlying procedure. While some, like the Copilot AI assistant in Microsoft Excel, do communicate the procedural steps in natural language, there is scope for including different ways to communicate more clearly to analysts (discussed more in Sec.~\ref{sec:discussion_impl_designers_semantics}). 
 

Based on our discussion, designing new AI-driven systems should also consider how to encourage users' adaptation to the procedure-oriented and data-oriented workflows. As new tools present a learning curve and unfamiliar elements, it is important to help analysts build comfort and confidence in various artifacts around different workflows.

% \subsubsection{Tools should clearly differentiate between deterministic and non-deterministic AI-generated artifacts}
% \label{sec:discussion_impl_designers_determinisitc}

% Participants (P4, P18, P21) sometimes expressed doubt on the intermediate data and even the summary visualizations as it was unclear to analysts what artifacts had the potential to be a result of AI hallucination~\cite{Ji2022SurveyOH} and what artifacts were consistent with regards to the data and procedure. This is especially pertinent as recent work~\cite{Dibia2023LIDAAT} and participants (P21, P22) in our study proposed AI-generated self-evaluations of its output to support evaluating and verifying AI-generations. As the line blurs between AI-generated artifacts and tool-generated artifacts, future tools should distinctly delineate between what is and is not AI-generated.

% For instance, this can be achieved through a side panel interface~\cite{Mcnutt2023OnTD} in which all of the deterministic elements are physically separated from the non-deterministic ones (like Fig.~\ref{fig:interface}). Similarly, communicating what parts of the process is AI-generated in creating an artifact is equally important. For instance, a tool presenting the summary visualizations in our study should communicate the underlying data was generated as part of the AI's procedure while the generation of the summary visualization is not. Clearly differentiating between components and the provenance of artifacts can help users gain confidence in the information from artifacts and better orientate themselves around the multitude of artifacts.

% \tim{the content very much seems to be about AI vs non AI generated while the title focuses on determinism. This felt like a mismatch to me. These seem like different things though AI generations often involve sampling, "temperature". The way you talk about it (e.g. hallucination) sounds like it puts a lot more weight on AI vs non AI.}


\subsubsection{Tools should support multiple ways to communicate the semantics of data operations}
\label{sec:discussion_impl_designers_semantics}
We observed AI-generated code to be a common part of analysts' verification processes in procedure-oriented and data-oriented workflows~(Sec.~\ref{sec:results_pworkflow} and Sec.~\ref{sec:results_dworkflow}). However, a lack of comprehension of the code and the exact data operations impacted analysts' confidence in their verification findings and even pushed them to alternative workflows~(Sec.~\ref{sec:results_bg_code}). However, participants who were able to translate the AI's code into familiar data operations were able to understand the procedure and not be significantly impacted in their verification confidence and process. Therefore, consistent with implications from prior work in XAI~\cite{Kim2022HelpMH}, tools should provide multiple methods to communicate the operations in the AI's procedure.

One example, mentioned by participants in our study is to translate the Python code into programming languages they were comfortable with. This can be achieved with neural code translators~\cite{Lachaux2020UnsupervisedTO} or existing AI-code assistants~\cite{ChatGPT, githubcopilot} at the code snippet level. 
% Given our discussion in Sec.~\ref{sec:discussion_impl_designers_determinisitc}, these translations should be clearly communicated as an AI-generated artifact. 
If translated at the operation level, it is important that the translation is faithful to the original operator. 

Besides communicating in different programming languages, Liu et al.~\cite{Liu2023WhatIW} explored translating Python code into a systematic natural language utterance and found this approach improved users' understanding of the code-generating model. However, this work only considered a limited set of operations and small data problems, and future work could explore how translating a larger set of operations could benefit analysts in real-world analysis tasks.

Tools can also leverage artifacts beyond code and natural language. Visualizations of data operations such as those in \textit{Datamations}~\cite{Pu2021DatamationsAE}, and \textit{SOMNUS}~\cite{Xiong2022VisualizingTS} can communicate operations visually to analysts. Likewise, tools can show differences in intermediate data between calculations to further enhance analysts' understanding of the operations~\cite{Wang2022DiffIT}.

\subsubsection{Tools should ask the AI to consistently communicate its assumptions and interpretations of the data}

We observed participants often noticed errors faster in tasks where the AI clearly stated its assumptions about the data (e.g., the data column semantics, assumed data types, and relationships between data columns etc.) and its interpretation of the prompt (P6, P10, P12, P22). For example, in T7, the AI clearly stated its interpretation of what the data in key columns represented: \shortquote{2021: (Assuming) Rank of the hotel in 2021} and \shortquote{Past\_rank: Past rank (unclear for which year).} However, we noticed similar assumptions were not always stated between different analysis tasks.

Therefore, tools should consistently communicate the assumptions and interpretations of the dataset and analysis, a well-regarded best practice for data analysis~\cite{Field2012DiscoveringSU}. This implication narrows down a broader recommendation for AI-based code assistants to articulate the generated code within the context of a programmer's specific task and environment~\cite{Sarkar2022WhatII}. One strategy to facilitate this could be to prompt the AI system to enumerate its assumptions explicitly. Another avenue, as exemplified by LLMs such as GPT-4 being good evaluators for tasks like natural language summarization and visualization~\cite{Dibia2023LIDAAT, Lin2022TeachingMT, Liu2023GEvalNE}, can involve employing a separate agent to evaluate the assistant-generated analysis, thereby listing any assumptions, interpretations, or discrepancies.


% \ken{could ask it to highlight}

% \tim{adding some example here to illustrate seems helpfful. what assumptions/interpretations are we talking about?}

% In traditional automatic data analytic paradigms, the emphasis has often been on evaluating the output—essentially, whether the tool and code delivers what it's supposed to. However, as we integrate large language models (LLMs) into increasingly complex workflows, such as data analysis verification processes, the focus is shifting. Our study reveals that analysts are actively engaged in understanding the AI's reasoning path and methodological approach. Specifically, our research highlights that analysts employ two predominant workflows—termed the \textbf{Procedure-Oriented Workflow} and the \textbf{Data-Oriented Workflow}—when verifying LLMs' data analysis output. In the \textbf{Procedure-Oriented Workflow}, analysts focused on understanding if all the steps are correctly conducted in correct procedure and logic. In contrast, the \textbf{Data-Oriented Workflow} focuses on the data inputs and outputs, scrutinizing their quality and relevance in the context of the task at hand. Rather than simply treating the AI as a 'black box' that either succeeds or fails in delivering the desired output, analysts are now actively validating the AI's reasoning process. This helps them gain a nuanced understanding of whether the AI system is adequately accomplishing its assigned tasks, thereby enhancing the trustworthiness of adopting AI's data analytics solution.

% We found that data plays a crucial role in the validation process. Participants made great use of the original data sets and intermediate data artifacts to verify the AI's analysis process. This suggests that data is not just an input or output in AI's data analysis, but an integral part of the validation process. 

% While the lack of programming language knowledge used to be a barrier in understanding analytics procedure \cite{}, our study demonstrated that code comments, explanations, and break down of steps generated by LLMs can effectively support participants understanding and verification process.

% We observed both data-oriented and procedure-oriented workflows in most data analysts, both are important. People don't just use one over the other, 

% \subsection{Design Opportunities}

% \xhdr{The need for integration with existing tool} With the rise of LLMs, there has been a discussion around whether we should build tools around LLMs or integrate LLMs into existing tools. Our findings highlight the need for AI's data analysis process to be integrated into users' existing tools. This would allow users to explore the intermediate steps of the AI's process and enhance their understanding of the analysis.

% \xhdr{Enhance users' familiarity with data operations and steps} While programming language is no longer a barrier, our study found that familiarity with data operations is still vital. This suggests that users need to have a good understanding of data operations to effectively verify the AI's data analysis process.

% \xhdr{Clearly delineate the sources of truth} A few participants expressed the preference of working with some source of truth, which could either be to executable code or the data tables. In addition to these, future systems could add more reliable reference points such as some built-in features to show data statistics and sanity check results for the user. Determining what is deterministic and predictable and non-deterministic.

% \xhdr{Prompt the LLMs to actively surface assumptions and identify potential issues (Self Evaluate)} We found that participants really appreciated when LLMs were able to find red flags in the result and suggest ways to fix the issue. However, among the task examples that we used in the study, LLMs made a few leaps in interpretation ambiguous data context, a behavior that our participant called out as \shortquote {lucky hallucination} (P22). Systems could prompt the LLMs to detect those communication ambiguities earlier on and ask for clarifications from the user to avoid making wrong assumptions. 



\subsection{Limitations and Future Work}
\label{sec:limitation}
We note several limitations in our study of verification processes and discuss opportunities for future work. First, the analysis task queries involved in our study tasks primarily involved sequences of data transformations. Other aspects of data analysis (e.g., data visualization, statistical modeling, machine learning, etc.) were not explored. However, our study still provided insight into analysis queries in common analysis workflows, as participants (P9, P22) mentioned the issues they encountered in the study tasks were ones they commonly faced in their own data analyses. Our study is a first step to uncovering verification processes  of AI-generated outputs where data and manipulations on data are centrally involved. Future work should explore analysts' verification processes in data visualization, statistical analysis, and machine learning workflows~\cite{Crisan2020PassingTD}.

Second, since our study contained a small number of verification tasks while using real responses generated by state-of-the-art nondeterministic models, components of the AI's explanation (e.g., listing its assumptions of the data and columns) and specific data operations involved in the data analysis task (i.e., filtering for data or merging data) were not controlled for across tasks. Future work could experiment with how varying components of the AI's explanation or analysis task impact analysts' verification processes. 

% Third, while our study elicited qualitative responses regarding participants' data and programming backgrounds, their are parts of their background that may influence the process we cannot quantify/capture. In particular, we could not identify the influences of AI-backgrounds on analysts' verification process. Given the infancy of AI-assisted data analysis tools, most participants in our study had not used AI assistance for analysis tasks. Future work could study analysts' verification workflows as they have increased exposure to these tools and an increased understanding of their error boundaries.

Third, participants were not the one's exploring the data and coming up with the analysis goal and instead had this given to them. As a result, prior to them verifying the AI-generated analyses, they first spent time understanding the data and analysis goal, a process that may not be as pertinent in conducting their own data analysis with AI assistants. However, to simulate realistic workflows, all tasks used in the study involved real-world datasets with analysis prompts written by data scientists (Sec.~\ref{sec:study}). In addition, we quickly clarified any questions regarding the analysis goal to facilitate the verification process. Future work could explore verification processes when analysts work with their own analysis tasks with the help of AI assistants. 

% \tim{verify my edits for accuracy -- you could refer back to your figure}
% \tim{However, all tasks were selected from ....--- make some argument why this decision was made, what benefits it may had. don't let the limitation linger too much on its own :) } 

Finally, study participants were not responsible for creating the AI prompts. While more elaborate prompts may be argued for reducing the errors presented in our study, writing these prompts is challenging~\cite{ZamfirescuPereira2023WhyJC, Mishra2022HELPMT}. Brevity of the prompt can be in tension with a precise one that reflects all aspects of the analysis~\cite{Yin2022NaturalLT}. 
% Formulating an unambiguous prompt is time-consuming, as even well-intentioned data analysts and participants in our own study expressed their needs in using AI to save time (P1, P13, P20). 
Therefore, given that the misalignment between the analyst's intent and AI's actions is inherent in natural language communication~\cite{Liu2023WhatIW, Luger2016LikeHA, zcan2020StateOT}, subtle AI-generated analysis errors (at least those due to this misalignment) and the need for verification processes persist. Moreover, as our study focuses on analysts' verification processes, we did not want LLM prompting expertise to impact and potentially bias the results. Recognizing errors remains a crucial aspect of Human-AI interaction, helping to enhance the quality of subsequent prompts for repair~\cite{Ashktorab2019ResilientCR} and future interactions. In a few cases, our participants (P6, P10, P22) noticed issues directly from language ambiguities in the intern's prompt. As a logical next step, future research should study how expertise in prompt creation influence analysts' interactions with AI assistants and how these analysts integrate prompts into their verification and repair strategies.











% prompts to be succint\ken{cite Ps?}. B




% \ken{if we talk about this then why even study human-ai in the first place if }


% Lab study and unfamiliar with the tool -> but we tried to mitigate with comprehensive tutorial, trial task, and relatively simple tool.
% Not doing their own analysis -> fundamental but real world analysis also now involves understanding the work of others and the work of other humans in collaboration with AI ~\cite{}

% Outside domain knowledge -> we tried out best to mitigate this



% Our work does not address those situations in which he fuzzy scenario where as people type more they can get a better understanding. due to our choice of not making it iteractive.


% In the post-task interview however, P8 later reflected that it was important to understand how the AI interprets the task requirement.

==> 8-discussion-future-work.tex <==
\section{Discussion}
\label{sec:discussion}
In this work, we examined how data analysts understand and verify AI-generated analyses. We developed a design probe, prepared realistic analysis queries and AI-generated analyses, and conducted a user study observing analysts' verification workflows and common behaviors. In this section, we synthesize the results from our user study and share implications for data analysts using AI-based analysis tools (Sec.~\ref{sec:discussion_impl_analyst}) and system designers building these tools (Sec.~\ref{sec:discussion_impl_designers}).


\subsection{Implications for Data Analysts}
\label{sec:discussion_impl_analyst}
\subsubsection{The Role of Data Literacy in Analysis Verification}
\label{sec:discussion_impl_analyst_data_lit}
Our findings suggest that while a lack of familiarity with one particular programming language (i.e., Python) is not a barrier for verifying AI-generated analyses, prior experience with data operations in other languages (e.g., SQL or Visual Basics for Applications) can aid in understanding the AI's procedure (Sec.~\ref{sec:results_bg_code}). Likewise, knowledge and experience in data analysis are often indispensable for grasping AI-generated analyses, mirroring the requirement for computational thinking skills when working with AI-based code assistants~\cite{Sarkar2022WhatII}. Here, we highlight two recommendations for analysts to be more effective in verifying AI-generated analyses.

% We found that even for experienced data scientists and analysts, they actively engage with both the procedure and datasets to identify the potential issues in AI's results (Sec.~\ref{sec:results}).

\yhdr{Know Common Data Operations} We observed participants closely examined the AI's data operations and sometimes performed these operations on the datasets directly to compare with AI's result (Secs.~\ref{sec:results_rq1_procedure_low} and~\ref{sec:results_rq2_data_support_procedure}). Their actions involved understanding common operations such as filtering, sorting, and merging the data. Similarly, understanding aggregation operations, such as sum, average, count, were essential to verify how the AI grouped data and performed calculations on those groups.

% In addition, analysts should also be familiar with some common ways to handle data quality issues. For example, in T10, the analyst should know ways of missing values to tell that the AI forgot to check the other columns which might contain values to fill in.

\yhdr{Develop Strategies for Quick Data Validations} Our observations revealed analysts often employed quick sanity checks on the data to assess AI-generated outputs (Secs.~\ref{sec:results_rq2_data} and ~\ref{sec:results_rq2_data_support_procedure}). Such strategies involved eyeballing values, manual summation of rows, using visualizations to check the value distributions, spot checking result values against original data table, and comparing things against common knowledge. These were effective for analysts to either build confidence in the results or identify unexpected patterns. The sanity checks often involved forming expectations around the result and then comparing them with the AI-generated output. Any discrepancies signaled potential issues that demanded further inspection. Given the effectiveness, analysts should actively identify quick sanity checks and externalize their expectations~\cite{Russell1993TheCS}. However, as there may be data issues hidden by seemingly reasonable patterns~\cite{correll2018looks}, analysts should employ a variety of different sanity checks.


\subsubsection{The Role of AI Assistants in Data Analysis}
\label{sec:discussion_impl_analyst_ai}

Participants' varied experiences working with data and analysis tools (Sec.~\ref{sec:results_bg}) led to a wide range of comments about their preferred use of general AI-based analysis assistants. Here, we discuss how AI assistants could be used in data analysis.

Some participants commented how AI-assistance would be helpful for getting them a partial answer that might guide them in their analysis (P1, P6, P7, P14, P20, P21). For instance, P6 mentioned how the AI can help them consider alternative steps: \shortquote{It'll help me say `oh maybe I didn't think of this way of solving this and I can now go down that path.'} AI assistants can help inspire ideas for analysis steps similar to when programmers follow an exploration mode in AI-assisted programming~\cite{Barke2022GroundedCH}. Presenting alternative approaches is especially critical in analysis assistance as analysts can often be limited in their consideration of analysis approaches~\cite{Liu2019PathsEP, Liu2020UnderstandingTR}, thereby affecting the robustness of their subsequent analysis conclusions~\cite{Silberzahn2018ManyAO, Breznau2022ObservingMR, Schweinsberg2021SameDD}. Thus, AI analysis assistance can improve analysis quality by broadening the analysis decision space analysts consider ~\cite{Liu2019PathsEP, Gu2022UnderstandingAS}. 
% \tim{you should cite your own multiverse paper :D}

Similarly, participants noted that assistants can expedite their analysis workflow (P1, P13, P20), corroborating the findings from prior research on AI-code assistants ~\cite{Vaithilingam2022ExpectationVE, Ziegler2022ProductivityAO, Dibia2022AligningOM, GitHubCopilotResearch}. However, to ensure the robustness of analysis conclusions, it is crucial to balance the acceleration of analysis with measures that surface potential errors, underlying data assumptions, and alternative approaches~\cite{Gu2023HowDD}.

Finally, some participants expressed a preference to reserve AI assistance for peripheral tasks such as error-checking or report generation rather than the central analysis. Utilizing AI assistance for crafting reports~\cite{Zheng2022TellingSF, Wang2023Slide4NCP} and similar subsidiary activities offers a low stakes environment for analysts to evaluate the quality of AI-generated outputs within data analysis workflows. Such use cases can also facilitate a deeper understanding of the assistant's capabilities and limitations.

\subsubsection{Understanding the Bounds of the AI and the Tool}

Participants sometimes expressed doubt on the intermediate data artifacts as it was unclear what artifacts had the potential to be a result of AI ``hallucinations"~\cite{Ji2022SurveyOH} and which were consistent with the data and procedure (Sec.~\ref{sec:results_bg_tools}). As the boundary blurs between AI-generated artifacts and tool-generated artifacts, analysts should clearly distinguish what is and what is not produced by AI.

Tool artifacts compiled from code is deterministic (i.e., the same summary visualization will be produced given the same code and input data)~\cite{Sarkar2022WhatII}. The AI-generated outputs and their associated errors are stochastic in nature, varying each time the AI is prompted to conduct the analysis. Knowing the provenance of artifacts used to support verification---what is tool-generated (e.g., the visual summary of data) and AI-generated (e.g., the intermediate data feeding into the visualization)---is important to assess the reliability of the information associated with these artifacts. Additionally, understanding the strengths and limitations of the AI~\cite{Ragavan2022GridBookNL, Sun2022InvestigatingEO} is crucial to knowing what types of mistakes to look for.


\subsection{Implications for System Designers}
Informed by our study findings of verification workflows and noted challenges, we highlight four design implications for designers of AI-based analysis assistants. 

\label{sec:discussion_impl_designers}
\subsubsection{Fluidly connecting data-oriented and procedure-oriented artifacts at various levels of granularity}
Our study on analysts' verification workflows indicated the use of data-oriented and procedure-oriented artifacts was often intimately tied to each other, requiring analysts to switch between the two (e.g., intermediate data table and the code snippet that generated this data). Therefore, tools should facilitate a seamless connection between the data and procedure. Integrating the data with the procedure aligns with existing implementations in data science and machine learning tools~\cite{Rahman2020LeamAI, Choi2023TowardsTR, Bauerle2022SymphonyCI, Kery2020mageFM, Wu2020B2BC}. Likewise, as analysts prefer different functionality based on their prior experiences (Sec.~\ref{sec:results_bg_tools}), data components should be interactive, reusable, and customizable to cater to specific preferences and applications~\cite{Bauerle2022SymphonyCI, Rahman2020LeamAI, Choi2023TowardsTR}. 


These connections should also prioritize verification behaviors. Participants often explored AI-generated analyses at different levels of abstraction (Secs. ~\ref{sec:results_rq1_procedure_high} and ~\ref{sec:results_rq1_procedure_low}) and transitioned between artifacts for quick glances of specific information (e.g., column names) or in-depth examinations involving multiple steps (Secs.~\ref{sec:results_rq2_data_support_procedure} and \ref{sec:results_rq2_procedure_support_data}). Therefore, tools should allow analysts to specify the scope of their current verification actions and surface the most relevant information. For example, when an analyst selects the text of a column name or cell value in the procedure, the tool can quickly highlight the corresponding data (and vice-versa). If the analyst selects a code snippet containing multiple data operations, the tool can highlight the corresponding data differences between the operations~\cite{Wang2022DiffIT}. Furthermore, to support analysts in tracing the data provenance of a given intermediate data (Sec.~\ref{sec:results_rq2_procedure_support_data}), the tool can highlight just the data operations in the procedure that produced it~\cite{Kery2017VarioliteSE, Head2019ManagingMI}. To support these features on the back-end, the AI can dynamically augment its text response to include semantically relevant connections to the data. Recent systems have demonstrated the efficacy of augmenting the AI's output for AI-assisted writing and exploration~\cite{Jiang2023GraphologueEL, Laban2023BeyondTC}. 

% \subsubsection{Tools should clearly differentiate between deterministic and non-deterministic AI-generated artifacts}
% \label{sec:discussion_impl_designers_determinisitc}

% Participants (P4, P18, P21) sometimes expressed doubt on the intermediate data and even the summary visualizations as it was unclear to analysts what artifacts had the potential to be a result of AI hallucination~\cite{Ji2022SurveyOH} and what artifacts were consistent with regards to the data and procedure. This is especially pertinent as recent work~\cite{Dibia2023LIDAAT} and participants (P21, P22) in our study proposed AI-generated self-evaluations of its output to support evaluating and verifying AI-generations. As the line blurs between AI-generated artifacts and tool-generated artifacts, future tools should distinctly delineate between what is and is not AI-generated.

% For instance, this can be achieved through a side panel interface~\cite{Mcnutt2023OnTD} in which all of the deterministic elements are physically separated from the non-deterministic ones (like Fig.~\ref{fig:interface}). Similarly, communicating what parts of the process is AI-generated in creating an artifact is equally important. For instance, a tool presenting the summary visualizations in our study should communicate the underlying data was generated as part of the AI's procedure while the generation of the summary visualization is not. Clearly differentiating between components and the provenance of artifacts can help users gain confidence in the information from artifacts and better orientate themselves around the multitude of artifacts.

% \tim{the content very much seems to be about AI vs non AI generated while the title focuses on determinism. This felt like a mismatch to me. These seem like different things though AI generations often involve sampling, "temperature". The way you talk about it (e.g. hallucination) sounds like it puts a lot more weight on AI vs non AI.}


\subsubsection{Communicating the semantics of data operations}
\label{sec:discussion_impl_designers_semantics}
We observed AI-generated code to be a common part of analysts' verification workflows in procedure-oriented and data-oriented behaviors~(Secs.~\ref{sec:results_rq2_procedure} and ~\ref{sec:results_rq2_procedure_support_data}). However, a lack of comprehension of the code and the exact data operations impacted analysts' confidence in their verification findings and even pushed them to alternative behaviors~(Sec.~\ref{sec:results_bg_code}). Nevertheless, participants who were able to translate the AI's code into familiar data operations were able to understand the procedure and not be significantly impacted. Therefore, consistent with implications from prior work~\cite{Kim2022HelpMH, Gu2023HowDD}, tools should provide multiple methods to communicate the operations in the AI's procedure.

For instance, participants suggested translating the Python code into programming languages they were comfortable with. This translation can be achieved with neural code translators~\cite{Lachaux2020UnsupervisedTO} or existing AI-code assistants~\cite{ChatGPT, githubcopilot} at the code snippet level. 
If translated at the operation level, it is essential to ensure faithfulness to the original operator. Alternatively, the code can be translated into systematic and consistent natural language utterances representing the data operations. On a limited set of operations and data problems, Liu et al.~\cite{Liu2023WhatIW}  found this approach improved users' understanding of the code-generating model. % Future work could explore how translating a larger set of operations could benefit analysts in real-world analysis tasks.
Additionally, besides code and natural language, tools can communicate data operations through visualizations such as those in \textit{Datamations}~\cite{Pu2021DatamationsAE}, and \textit{SOMNUS}~\cite{Xiong2022VisualizingTS}. Likewise, tools can show differences in intermediate data between calculations to further enhance analysts' understanding of the operations~\cite{Wang2022DiffIT}.


\subsubsection{Communicating AI's assumptions and interpretations of the data}

We observed participants often noticed errors faster in tasks where the AI clearly stated its assumptions about the data (e.g., the data column semantics, assumed data types, and relationships between data columns etc.) and its interpretation of the prompt (P6, P10, P12, P22). For example, in T7, the AI clearly stated its interpretation of what the data in key columns represented: \shortquote{2021: (Assuming) Rank of the hotel in 2021} and \shortquote{Past\_rank: Past rank (unclear for which year).} However, we noticed similar assumptions were not always stated in other tasks.

Therefore, tools should consistently communicate the assumptions and interpretations of the dataset and analysis, a well-regarded best practice for data analysis~\cite{Field2012DiscoveringSU}. This implication narrows down a broader recommendation for AI-based code assistants to articulate the generated code within the context of a programmer's specific task and environment~\cite{Sarkar2022WhatII}. One strategy to facilitate regular communication could be to prompt the AI system to enumerate its assumptions explicitly. Another avenue, as exemplified by LLMs such as GPT-4 being good evaluators for tasks like natural language summarization and visualization~\cite{Dibia2023LIDAAT, Lin2022TeachingMT, Liu2023GEvalNE}, can involve employing a separate agent to evaluate the assistant-generated analysis, thereby listing any assumptions, interpretations, or discrepancies.

 
\subsubsection{Incorporating AI guidance into verification workflows}
In a world where AI can generate data analyses, analysis verification becomes an increasingly important skill~\cite{Tu2023WhatSD}. In our study, we noticed variations in participants' verification approaches, with more experienced participants proactively formulating systematic plans (Sec.~\ref{sec:results_bg_data}). As LLMs show promise for making data analysis approachable to broader audiences, there is an opportunity for tools to guide analysts in their verification workflows. 

For example, to help with quick data checks (Sec.~\ref{sec:results_rq2_data_support_procedure}), LLMs can generate test cases. For instance, if a field represents age, then only values between 0 and around 120 might be appropriate. Furthermore, identifying missing values (which might be 0) might help in the analysis process. However, different than prior work where generated test cases were for general programming problems ~\cite{Tufano2020UnitTC, Chen2022CodeTCG}, test cases for data analyses need to consider the semantics and domain of the data. Specifically, as outputs from data analysis are meant for human understanding and involve complex data structures
(e.g., data tables, plots), there can be alternative ways to present the answer (e.g., different views of the same data table)~\cite{Yin2022NaturalLT, Lai2022DS1000AN, Huang2022ExecutionbasedEF}. Likewise, since AI-generated analyses can involve sequences of data operations, it is pertinent to create test cases for both the final output and intermediate steps.

Additionally, as a key part of verification involves checking for inconsistencies (Sec.~\ref{sec:results_rq2_procedure}), our findings suggest opportunities for AI self-reflection~\cite{Jiang2023SelfEvolveAC, Shinn2023ReflexionAA, Park2023GenerativeAI, Sumers2023CognitiveAF} to help analysts identify potential discrepancies, formulate specific checklists, and improve their data literacy (Sec.~\ref{sec:discussion_impl_analyst_data_lit}). This reflection should be contextualized with external knowledge of existing best analysis practices and the contents of the working analysis. In incorporating AI self-reflection, the interface can visually highlight specific sections of the analysis that require verification. Such visual warnings can help reduce analysts' overconfidence in the AI's procedures~\cite{Laban2023BeyondTC}. However, given the failure modes of LLMs~\cite{Bender2021OnTD, Ji2022SurveyOH}, it is crucial to communicate to the analyst the parts of guidance that are AI generated.





% \ken{could ask it to highlight}

% \tim{adding some example here to illustrate seems helpfful. what assumptions/interpretations are we talking about?}

% In traditional automatic data analytic paradigms, the emphasis has often been on evaluating the output—essentially, whether the tool and code delivers what it's supposed to. However, as we integrate large language models (LLMs) into increasingly complex workflows, such as data analysis verification processes, the focus is shifting. Our study reveals that analysts are actively engaged in understanding the AI's reasoning path and methodological approach. Specifically, our research highlights that analysts employ two predominant workflows—termed the \textbf{Procedure-Oriented Workflow} and the \textbf{Data-Oriented Workflow}—when verifying LLMs' data analysis output. In the \textbf{Procedure-Oriented Workflow}, analysts focused on understanding if all the steps are correctly conducted in correct procedure and logic. In contrast, the \textbf{Data-Oriented Workflow} focuses on the data inputs and outputs, scrutinizing their quality and relevance in the context of the task at hand. Rather than simply treating the AI as a 'black box' that either succeeds or fails in delivering the desired output, analysts are now actively validating the AI's reasoning process. This helps them gain a nuanced understanding of whether the AI system is adequately accomplishing its assigned tasks, thereby enhancing the trustworthiness of adopting AI's data analytics solution.

% We found that data plays a crucial role in the validation process. Participants made great use of the original data sets and intermediate data artifacts to verify the AI's analysis process. This suggests that data is not just an input or output in AI's data analysis, but an integral part of the validation process. 

% While the lack of programming language knowledge used to be a barrier in understanding analytics procedure \cite{}, our study demonstrated that code comments, explanations, and break down of steps generated by LLMs can effectively support participants understanding and verification process.

% We observed both data-oriented and procedure-oriented workflows in most data analysts, both are important. People don't just use one over the other, 

% \subsection{Design Opportunities}

% \xhdr{The need for integration with existing tool} With the rise of LLMs, there has been a discussion around whether we should build tools around LLMs or integrate LLMs into existing tools. Our findings highlight the need for AI's data analysis process to be integrated into users' existing tools. This would allow users to explore the intermediate steps of the AI's process and enhance their understanding of the analysis.

% \xhdr{Enhance users' familiarity with data operations and steps} While programming language is no longer a barrier, our study found that familiarity with data operations is still vital. This suggests that users need to have a good understanding of data operations to effectively verify the AI's data analysis process.

% \xhdr{Clearly delineate the sources of truth} A few participants expressed the preference of working with some source of truth, which could either be to executable code or the data tables. In addition to these, future systems could add more reliable reference points such as some built-in features to show data statistics and sanity check results for the user. Determining what is deterministic and predictable and non-deterministic.

% \xhdr{Prompt the LLMs to actively surface assumptions and identify potential issues (Self Evaluate)} We found that participants really appreciated when LLMs were able to find red flags in the result and suggest ways to fix the issue. However, among the task examples that we used in the study, LLMs made a few leaps in interpretation ambiguous data context, a behavior that our participant called out as \shortquote {lucky hallucination} (P22). Systems could prompt the LLMs to detect those communication ambiguities earlier on and ask for clarifications from the user to avoid making wrong assumptions. 



\subsection{Limitations and Future Work}
\label{sec:limitation}
We note several limitations in our study and discuss opportunities for future work. 

First, the analysis queries involved in the study tasks primarily involved sequences of data transformations. Other aspects of data analysis (e.g., data visualization, statistical modeling, machine learning, etc.) were not explored. However, our study still provided insight into common analysis workflows, as participants (P9, P22) mentioned the issues they encountered in the study tasks were ones they commonly faced in their own data analyses. Our study is a first step towards uncovering verification workflows of AI-generated outputs where data and manipulations on data are centrally involved. Future work should explore analysts' verification of AI-generated data visualizations, statistical analyses, and machine learning pipelines~\cite{Crisan2020PassingTD}.

Second, since our study contained a small number of verification tasks while using real responses generated by state-of-the-art nondeterministic models, components of the AI's explanation (e.g., listing its assumptions of the data and columns) and specific data operations involved in the data analysis task (i.e., filtering for data or merging data) were not controlled for across tasks. Future work could experiment with how varying components of the AI's explanation or analysis task impact analysts' verification processes. 

% Third, while our study elicited qualitative responses regarding participants' data and programming backgrounds, their are parts of their background that may influence the process we cannot quantify/capture. In particular, we could not identify the influences of AI-backgrounds on analysts' verification process. Given the infancy of AI-assisted data analysis tools, most participants in our study had not used AI assistance for analysis tasks. Future work could study analysts' verification workflows as they have increased exposure to these tools and an increased understanding of their error boundaries.

Third, as discussed in our study desisgn considerations (Sec.~\ref{sec:method_design}) participants were not the ones gathering the data and coming up with the analysis goal. As a result, prior to them verifying the AI-generated analyses, they first spent time understanding the data and analysis goal, a process that may not be as pertinent in conducting their own data analysis with AI assistants. However, all tasks used in the study involved real-world datasets with analysis prompts written by data scientists (Sec.~\ref{sec:study}). In addition, we quickly clarified any questions regarding the analysis goal to facilitate analysts' verification. Future work could explore verification workflows when analysts work with an AI assistant on their own data and analysis. 


Finally, study participants were not responsible for creating the AI prompts (Sec.~\ref{sec:method_design}). While more elaborate prompts may be argued for reducing the errors presented in our study, writing these prompts is challenging~\cite{ZamfirescuPereira2023WhyJC, Mishra2022HELPMT}. Brevity of the prompt can be in tension with a precise one that reflects all aspects of the analysis~\cite{Yin2022NaturalLT}. 
% Formulating an unambiguous prompt is time-consuming, as even well-intentioned data analysts and participants in our own study expressed their needs in using AI to save time (P1, P13, P20). 
Therefore, given that the misalignment between the analyst's intent and AI's actions is inherent in natural language communication~\cite{Liu2023WhatIW, Luger2016LikeHA, zcan2020StateOT}, subtle AI-generated analysis errors (at least those due to misalignment) and the need for verification workflows persist. 
% Moreover, as our study focuses on analysts' verification processes, we did not want LLM prompting expertise to impact and potentially bias the results. 
% Recognizing errors remains a crucial aspect of Human-AI interaction, helping to enhance the quality of subsequent prompts for repair~\cite{Ashktorab2019ResilientCR} and future interactions.
In a few cases, our participants (P6, P10, P22) noticed issues directly from language ambiguities in the intern's prompt. As a logical next step, future research should study how expertise in prompt writing influence analysts' interactions with AI assistants and how these analysts integrate prompts into their verification and repair strategies.











% prompts to be succint\ken{cite Ps?}. B




% \ken{if we talk about this then why even study human-ai in the first place if }


% Lab study and unfamiliar with the tool -> but we tried to mitigate with comprehensive tutorial, trial task, and relatively simple tool.
% Not doing their own analysis -> fundamental but real world analysis also now involves understanding the work of others and the work of other humans in collaboration with AI ~\cite{}

% Outside domain knowledge -> we tried out best to mitigate this



% Our work does not address those situations in which he fuzzy scenario where as people type more they can get a better understanding. due to our choice of not making it iteractive.


% In the post-task interview however, P8 later reflected that it was important to understand how the AI interprets the task requirement.

==> 9-conclusion.tex <==
\section{Conclusion}
%\anna{TODO}
In this paper, we explore data analysts' behaviors when verifying AI-generated analyses. We build a design probe and prepare tasks with realistic analysis intent and LLM outputs generated by OpenAI's Code Interpreter. In a controlled user study, we find analysts frequently interleaved \textit{procedure-oriented} and \textit{data-oriented behaviors}, using data artifacts in support of \processworkflows and procedure artifacts in support of their \dataworkflows. We also find analysts' prior analysis and programming experiences influenced their approach and understanding of the AI's output. Based on our findings, we synthesize recommendations for data analysts and highlight opportunities for future tools to enhance the verification experience, including communicating the AI's assumptions and interpretations of the data, and ways to incorporate AI guidance in verification workflows.




%the potential of AI-based data analysis assistants that incorporate execution and planning assistance. To understand the space of helpful suggestions, we perform a \litreview review and a behavior-driven study to establish a categorization of analysis suggestions. To explore the essential components of a helpful suggestion, we design and conduct a \woz study that is inspired by but not limited by the capabilities of existing LLM-based assistants. This work contributes the first user study involving analysts working on a real dataset and task to better understand how to design and incorporate planning assistance into analysts' workflows. In addition, we provide an open-source implementation of an assistant interface building on prior work. From our study, we find that analysts found many categories of planning assistance helpful, highlighting the potential of incorporating planning assistance. However, in order to achieve this, it is crucial to comprehend and address the contextual factors that influence analysts' willingness to consider planning suggestions. We synthesize these findings to highlight design implications for future AI-based analysis assistants. Among these are aligning the analysis and the assistant on shared analysis goals and adding measures to reduce overreliance and promote trust 
% \tim{what could we say here to be  more specific about engagement? promote trust but not overreliance? etc?}in this new analyst-assistant paradigm. 

%\ken{TODO}
